Distance-critical and distance-redundant graphs

If a vertex in a graph can be deleted without affecting distances among the other vertices, we shall say it is distance-redundant. Graphs with all, some or no such vertices are discussed. (The latter class was termed distance-critical by Erd\H{o}s and Howorka).

==> Gnp100.tex <==
\begin{semilogyaxis}[
xmin= 0, xmax= 0.5,
xlabel={$p$},
ylabel={num vertices, $D$},
ylabel near ticks,
]
\addplot [red]
coordinates {
( 0.03, 15.943396)
( 0.03755102, 10.9725)
( 0.045102041, 7.5775)
( 0.052653061, 4.9125)
( 0.060204082, 3.5675)
( 0.067755102, 2.365)
( 0.075306122, 1.6125)
( 0.082857143, 1.2625)
( 0.090408163, 0.98)
( 0.097959184, 0.7625)
( 0.1055102, 0.6725)
( 0.11306122, 0.7125)
( 0.12061224, 0.6525)
( 0.12816327, 0.68)
( 0.13571429, 0.87)
( 0.14326531, 1.035)
( 0.15081633, 1.2)
( 0.15836735, 1.6925)
( 0.16591837, 2.4625)
( 0.17346939, 3.585)
( 0.18102041, 5.45)
( 0.18857143, 7.75)
( 0.19612245, 11.245)
( 0.20367347, 16.325)
( 0.21122449, 23.08)
( 0.21877551, 29.9125)
( 0.22632653, 39.1325)
( 0.23387755, 48.1325)
( 0.24142857, 57.795)
( 0.24897959, 66.56)
( 0.25653061, 74.7025)
( 0.26408163, 80.8875)
( 0.27163265, 86.2425)
( 0.27918367, 90.865)
( 0.28673469, 93.395)
( 0.29428571, 95.7275)
( 0.30183673, 97.1425)
( 0.30938776, 98.225)
( 0.31693878, 98.84)
( 0.3244898, 99.265)
( 0.33204082, 99.62)
( 0.33959184, 99.7425)
( 0.34714286, 99.8575)
( 0.35469388, 99.905)
( 0.3622449, 99.9725)
( 0.36979592, 99.975)
( 0.37734694, 99.98)
( 0.38489796, 99.99)
( 0.39244898, 99.9925)
( 0.4, 99.9925)
( 0.6, 100)
( 0.8, 100)
( 0.99, 100)
};
\addplot [dashed]
coordinates {
( 0.03, 8.8113208)
( 0.03755102, 7.5325)
( 0.045102041, 6.515)
( 0.052653061, 5.815)
( 0.060204082, 5.295)
( 0.067755102, 4.9)
( 0.075306122, 4.435)
( 0.082857143, 4.1625)
( 0.090408163, 4.0325)
( 0.097959184, 3.9975)
( 0.1055102, 3.875)
( 0.11306122, 3.6575)
( 0.12061224, 3.35)
( 0.12816327, 3.1475)
( 0.13571429, 3.0625)
( 0.14326531, 3.015)
( 0.15081633, 3.005)
( 0.15836735, 3.0025)
( 0.16591837, 3.005)
( 0.17346939, 3)
( 0.18102041, 3)
( 0.18857143, 3)
( 0.19612245, 3)
( 0.20367347, 3)
( 0.21122449, 3)
( 0.21877551, 3)
( 0.22632653, 3)
( 0.23387755, 3)
( 0.24142857, 3)
( 0.24897959, 2.99)
( 0.25653061, 2.96)
( 0.26408163, 2.91)
( 0.27163265, 2.7825)
( 0.27918367, 2.63)
( 0.28673469, 2.4725)
( 0.29428571, 2.385)
( 0.30183673, 2.2175)
( 0.30938776, 2.1575)
( 0.31693878, 2.0625)
( 0.3244898, 2.0625)
( 0.33204082, 2.055)
( 0.33959184, 2.0125)
( 0.34714286, 2.0125)
( 0.35469388, 2.0075)
( 0.3622449, 2.0025)
( 0.36979592, 2.0025)
( 0.37734694, 2.0025)
( 0.38489796, 2)
( 0.39244898, 2)
( 0.4, 2)
( 0.6, 2)
( 0.8, 2)
( 0.99, 2)
};
\addplot [blue,dash dot]
coordinates {
( 0.03, 26.415094)
( 0.03755102, 25.76)
( 0.045102041, 34.4825)
( 0.052653061, 52.63)
( 0.060204082, 72.18)
( 0.067755102, 89.1225)
( 0.075306122, 96.5725)
( 0.082857143, 99.1775)
( 0.090408163, 99.795)
( 0.097959184, 99.975)
( 0.1055102, 99.9925)
( 0.11306122, 99.9975)
( 0.12061224, 100)
( 0.12816327, 100)
( 0.13571429, 100)
( 0.14326531, 100)
( 0.15081633, 100)
( 0.15836735, 100)
( 0.16591837, 100)
( 0.17346939, 100)
( 0.18102041, 100)
( 0.18857143, 100)
( 0.19612245, 100)
( 0.20367347, 100)
( 0.21122449, 100)
( 0.21877551, 100)
( 0.22632653, 100)
( 0.23387755, 100)
( 0.24142857, 100)
( 0.24897959, 100)
( 0.25653061, 100)
( 0.26408163, 100)
( 0.27163265, 100)
( 0.27918367, 100)
( 0.28673469, 100)
( 0.29428571, 100)
( 0.30183673, 100)
( 0.30938776, 100)
( 0.31693878, 100)
( 0.3244898, 100)
( 0.33204082, 100)
( 0.33959184, 100)
( 0.34714286, 100)
( 0.35469388, 100)
( 0.3622449, 100)
( 0.36979592, 100)
( 0.37734694, 100)
( 0.38489796, 100)
( 0.39244898, 100)
( 0.4, 100)
( 0.6, 100)
( 0.8, 100)
( 0.99, 100)
};
\addplot [red,dotted]
coordinates {
( 0.01, 75.0269435)
( 0.0111823647, 70.9435795)
( 0.0123647295, 66.9132973)
( 0.0135470942, 62.9745354)
( 0.0147294589, 59.1560832)
( 0.0159118236, 55.4787952)
( 0.0170941884, 51.9570462)
( 0.0182765531, 48.5999647)
( 0.0194589178, 45.4124714)
( 0.0206412826, 42.3961507)
( 0.0218236473, 39.5499777)
( 0.023006012, 36.8709222)
( 0.0241883768, 34.3544469)
( 0.0253707415, 31.9949149)
( 0.0265531062, 29.7859223)
( 0.0277354709, 27.7205651)
( 0.0289178357, 25.7916531)
( 0.0301002004, 23.9918782)
( 0.0312825651, 22.313945)
( 0.0324649299, 20.7506707)
( 0.0336472946, 19.2950598)
( 0.0348296593, 17.9403576)
( 0.036012024, 16.6800876)
( 0.0371943888, 15.5080751)
( 0.0383767535, 14.4184607)
( 0.0395591182, 13.4057056)
( 0.040741483, 12.4645904)
( 0.0419238477, 11.5902093)
( 0.0431062124, 10.7779611)
( 0.0442885772, 10.023538)
( 0.0454709419, 9.32291177)
( 0.0466533066, 8.6723206)
( 0.0478356713, 8.0682541)
( 0.0490180361, 7.507439)
( 0.0502004008, 6.98682482)
( 0.0513827655, 6.50356993)
( 0.0525651303, 6.05502821)
( 0.053747495, 5.63873625)
( 0.0549298597, 5.25240126)
( 0.0561122244, 4.89388968)
( 0.0572945892, 4.56121644)
( 0.0584769539, 4.25253494)
( 0.0596593186, 3.96612762)
( 0.0608416834, 3.70039721)
( 0.0620240481, 3.45385851)
( 0.0632064128, 3.22513081)
( 0.0643887776, 3.0129307)
( 0.0655711423, 2.81606547)
( 0.066753507, 2.63342689)
( 0.0679358717, 2.46398548)
( 0.0691182365, 2.30678504)
( 0.0703006012, 2.16093772)
( 0.0714829659, 2.02561923)
( 0.0726653307, 1.90006454)
( 0.0738476954, 1.78356376)
( 0.0750300601, 1.6754583)
( 0.0762124248, 1.57513738)
( 0.0773947896, 1.48203462)
( 0.0785771543, 1.39562502)
( 0.079759519, 1.31542201)
( 0.0809418838, 1.24097477)
( 0.0821242485, 1.17186575)
( 0.0833066132, 1.10770825)
( 0.084488978, 1.04814429)
( 0.0856713427, 0.992842577)
( 0.0868537074, 0.941496557)
( 0.0880360721, 0.893822701)
( 0.0892184369, 0.849558835)
( 0.0904008016, 0.808462621)
( 0.0915831663, 0.770310131)
( 0.0927655311, 0.734894528)
( 0.0939478958, 0.702024843)
( 0.0951302605, 0.671524835)
( 0.0963126253, 0.643231937)
( 0.09749499, 0.616996279)
( 0.0986773547, 0.592679784)
( 0.0998597194, 0.570155329)
( 0.101042084, 0.549305974)
( 0.102224449, 0.53002425)
( 0.103406814, 0.512211497)
( 0.104589178, 0.495777264)
( 0.105771543, 0.480638752)
( 0.106953908, 0.466720302)
( 0.108136273, 0.453952935)
( 0.109318637, 0.44227392)
( 0.110501002, 0.431626396)
( 0.111683367, 0.421959017)
( 0.112865731, 0.413225643)
( 0.114048096, 0.405385052)
( 0.115230461, 0.398400699)
( 0.116412826, 0.392240489)
( 0.11759519, 0.386876593)
( 0.118777555, 0.382285282)
( 0.11995992, 0.378446797)
( 0.121142285, 0.375345236)
( 0.122324649, 0.372968481)
( 0.123507014, 0.371308134)
( 0.124689379, 0.3703595)
( 0.125871743, 0.370121574)
( 0.127054108, 0.370597076)
( 0.128236473, 0.371792495)
( 0.129418838, 0.373718178)
( 0.130601202, 0.376388433)
( 0.131783567, 0.379821673)
( 0.132965932, 0.384040588)
( 0.134148297, 0.389072349)
( 0.135330661, 0.394948851)
( 0.136513026, 0.401706989)
( 0.137695391, 0.40938898)
( 0.138877756, 0.418042723)
( 0.14006012, 0.427722203)
( 0.141242485, 0.438487955)
( 0.14242485, 0.450407562)
( 0.143607214, 0.46355623)
( 0.144789579, 0.478017406)
( 0.145971944, 0.493883472)
( 0.147154309, 0.511256502)
( 0.148336673, 0.530249095)
( 0.149519038, 0.550985287)
( 0.150701403, 0.573601545)
( 0.151883768, 0.598247853)
( 0.153066132, 0.625088885)
( 0.154248497, 0.654305283)
( 0.155430862, 0.686095036)
( 0.156613226, 0.720674956)
( 0.157795591, 0.758282281)
( 0.158977956, 0.799176371)
( 0.160160321, 0.84364053)
( 0.161342685, 0.891983934)
( 0.16252505, 0.944543671)
( 0.163707415, 1.00168689)
( 0.16488978, 1.06381303)
( 0.166072144, 1.1313562)
( 0.167254509, 1.20478751)
( 0.168436874, 1.28461764)
( 0.169619238, 1.37139927)
( 0.170801603, 1.46572964)
( 0.171983968, 1.56825304)
( 0.173166333, 1.67966326)
( 0.174348697, 1.80070595)
( 0.175531062, 1.93218077)
( 0.176713427, 2.07494345)
( 0.177895792, 2.22990747)
( 0.179078156, 2.39804545)
( 0.180260521, 2.58039014)
( 0.181442886, 2.77803494)
( 0.182625251, 2.99213374)
( 0.183807615, 3.22390025)
( 0.18498998, 3.47460646)
( 0.186172345, 3.74558032)
( 0.187354709, 4.03820248)
( 0.188537074, 4.35390205)
( 0.189719439, 4.69415122)
( 0.190901804, 5.06045882)
( 0.192084168, 5.45436265)
( 0.193266533, 5.8774206)
( 0.194448898, 6.33120058)
( 0.195631263, 6.81726915)
( 0.196813627, 7.3371791)
( 0.197995992, 7.89245583)
( 0.199178357, 8.48458279)
( 0.200360721, 9.11498599)
( 0.201543086, 9.78501785)
( 0.202725451, 10.4959405)
( 0.203907816, 11.2489087)
( 0.20509018, 12.044953)
( 0.206272545, 12.8849625)
( 0.20745491, 13.7696689)
( 0.208637275, 14.6996304)
( 0.209819639, 15.6752176)
( 0.211002004, 16.6966)
( 0.212184369, 17.7637346)
( 0.213366733, 18.876356)
( 0.214549098, 20.033969)
( 0.215731463, 21.2358435)
( 0.216913828, 22.4810113)
( 0.218096192, 23.7682662)
( 0.219278557, 25.0961666)
( 0.220460922, 26.4630404)
( 0.221643287, 27.866993)
( 0.222825651, 29.3059176)
( 0.224008016, 30.7775081)
( 0.225190381, 32.2792742)
( 0.226372745, 33.8085585)
( 0.22755511, 35.3625551)
( 0.228737475, 36.9383305)
( 0.22991984, 38.5328449)
( 0.231102204, 40.1429745)
( 0.232284569, 41.7655346)
( 0.233466934, 43.3973031)
( 0.234649299, 45.035043)
( 0.235831663, 46.6755253)
( 0.237014028, 48.3155513)
( 0.238196393, 49.951973)
( 0.239378758, 51.5817133)
( 0.240561122, 53.2017843)
( 0.241743487, 54.8093039)
( 0.242925852, 56.4015114)
( 0.244108216, 57.9757805)
( 0.245290581, 59.5296309)
( 0.246472946, 61.0607379)
( 0.247655311, 62.5669402)
( 0.248837675, 64.0462458)
( 0.25002004, 65.4968359)
( 0.251202405, 66.9170676)
( 0.25238477, 68.3054744)
( 0.253567134, 69.6607657)
( 0.254749499, 70.9818243)
( 0.255931864, 72.2677035)
( 0.257114228, 73.5176221)
( 0.258296593, 74.7309594)
( 0.259478958, 75.9072484)
( 0.260661323, 77.046169)
( 0.261843687, 78.1475405)
( 0.263026052, 79.2113131)
( 0.264208417, 80.2375602)
( 0.265390782, 81.2264691)
( 0.266573146, 82.1783327)
( 0.267755511, 83.0935405)
( 0.268937876, 83.97257)
( 0.27012024, 84.8159784)
( 0.271302605, 85.6243935)
( 0.27248497, 86.3985066)
( 0.273667335, 87.1390636)
( 0.274849699, 87.8468584)
( 0.276032064, 88.522725)
( 0.277214429, 89.1675316)
( 0.278396794, 89.7821734)
( 0.279579158, 90.3675671)
( 0.280761523, 90.9246454)
( 0.281943888, 91.4543517)
( 0.283126253, 91.9576354)
( 0.284308617, 92.4354478)
( 0.285490982, 92.8887378)
( 0.286673347, 93.3184488)
( 0.287855711, 93.7255154)
( 0.289038076, 94.1108602)
( 0.290220441, 94.4753917)
( 0.291402806, 94.8200021)
( 0.29258517, 95.1455652)
( 0.293767535, 95.4529349)
( 0.2949499, 95.7429439)
( 0.296132265, 96.0164022)
( 0.297314629, 96.2740967)
( 0.298496994, 96.5167903)
( 0.299679359, 96.745221)
( 0.300861723, 96.9601022)
( 0.302044088, 97.1621218)
( 0.303226453, 97.3519426)
( 0.304408818, 97.5302023)
( 0.305591182, 97.6975132)
( 0.306773547, 97.854463)
( 0.307955912, 98.0016149)
( 0.309138277, 98.1395077)
( 0.310320641, 98.268657)
( 0.311503006, 98.3895547)
( 0.312685371, 98.5026706)
( 0.313867735, 98.6084521)
( 0.3150501, 98.7073255)
( 0.316232465, 98.7996962)
( 0.31741483, 98.8859496)
( 0.318597194, 98.9664517)
( 0.319779559, 99.0415496)
( 0.320961924, 99.1115727)
( 0.322144289, 99.1768329)
( 0.323326653, 99.2376253)
( 0.324509018, 99.2942293)
( 0.325691383, 99.3469088)
( 0.326873747, 99.3959132)
( 0.328056112, 99.4414777)
( 0.329238477, 99.4838244)
( 0.330420842, 99.5231625)
( 0.331603206, 99.559689)
( 0.332785571, 99.5935894)
( 0.333967936, 99.6250384)
( 0.335150301, 99.6542)
( 0.336332665, 99.6812283)
( 0.33751503, 99.7062683)
( 0.338697395, 99.7294556)
( 0.33987976, 99.7509179)
( 0.341062124, 99.7707746)
( 0.342244489, 99.7891375)
( 0.343426854, 99.8061115)
( 0.344609218, 99.8217946)
( 0.345791583, 99.8362786)
( 0.346973948, 99.8496493)
( 0.348156313, 99.8619866)
( 0.349338677, 99.8733654)
( 0.350521042, 99.8838556)
( 0.351703407, 99.8935222)
( 0.352885772, 99.9024259)
( 0.354068136, 99.9106233)
( 0.355250501, 99.918167)
( 0.356432866, 99.9251062)
( 0.35761523, 99.9314864)
( 0.358797595, 99.93735)
( 0.35997996, 99.9427365)
( 0.361162325, 99.9476824)
( 0.362344689, 99.9522218)
( 0.363527054, 99.9563863)
( 0.364709419, 99.9602051)
( 0.365891784, 99.9637052)
( 0.367074148, 99.966912)
( 0.368256513, 99.9698486)
( 0.369438878, 99.9725366)
( 0.370621242, 99.9749959)
( 0.371803607, 99.977245)
( 0.372985972, 99.9793009)
( 0.374168337, 99.9811794)
( 0.375350701, 99.982895)
( 0.376533066, 99.984461)
( 0.377715431, 99.98589)
( 0.378897796, 99.9871933)
( 0.38008016, 99.9883814)
( 0.381262525, 99.9894639)
( 0.38244489, 99.9904499)
( 0.383627255, 99.9913475)
( 0.384809619, 99.9921643)
( 0.385991984, 99.9929072)
( 0.387174349, 99.9935826)
( 0.388356713, 99.9941963)
( 0.389539078, 99.9947537)
( 0.390721443, 99.9952597)
( 0.391903808, 99.9957189)
( 0.393086172, 99.9961353)
( 0.394268537, 99.9965129)
( 0.395450902, 99.996855)
( 0.396633267, 99.9971649)
( 0.397815631, 99.9974454)
( 0.398997996, 99.9976993)
( 0.400180361, 99.9979289)
( 0.401362725, 99.9981364)
( 0.40254509, 99.9983239)
( 0.403727455, 99.9984933)
( 0.40490982, 99.9986462)
( 0.406092184, 99.9987841)
( 0.407274549, 99.9989086)
( 0.408456914, 99.9990207)
( 0.409639279, 99.9991217)
( 0.410821643, 99.9992127)
( 0.412004008, 99.9992946)
( 0.413186373, 99.9993683)
( 0.414368737, 99.9994346)
( 0.415551102, 99.9994942)
( 0.416733467, 99.9995477)
( 0.417915832, 99.9995957)
( 0.419098196, 99.9996388)
( 0.420280561, 99.9996775)
( 0.421462926, 99.9997122)
( 0.422645291, 99.9997432)
( 0.423827655, 99.9997711)
( 0.42501002, 99.999796)
( 0.426192385, 99.9998183)
( 0.427374749, 99.9998382)
( 0.428557114, 99.999856)
( 0.429739479, 99.999872)
( 0.430921844, 99.9998862)
( 0.432104208, 99.9998989)
( 0.433286573, 99.9999102)
( 0.434468938, 99.9999203)
( 0.435651303, 99.9999293)
( 0.436833667, 99.9999373)
( 0.438016032, 99.9999444)
( 0.439198397, 99.9999508)
( 0.440380762, 99.9999564)
( 0.441563126, 99.9999614)
( 0.442745491, 99.9999659)
( 0.443927856, 99.9999699)
( 0.44511022, 99.9999734)
( 0.446292585, 99.9999765)
( 0.44747495, 99.9999792)
( 0.448657315, 99.9999817)
( 0.449839679, 99.9999839)
( 0.451022044, 99.9999858)
( 0.452204409, 99.9999875)
( 0.453386774, 99.999989)
( 0.454569138, 99.9999903)
( 0.455751503, 99.9999915)
( 0.456933868, 99.9999925)
( 0.458116232, 99.9999934)
( 0.459298597, 99.9999942)
( 0.460480962, 99.9999949)
( 0.461663327, 99.9999956)
( 0.462845691, 99.9999961)
( 0.464028056, 99.9999966)
( 0.465210421, 99.999997)
( 0.466392786, 99.9999974)
( 0.46757515, 99.9999977)
( 0.468757515, 99.999998)
( 0.46993988, 99.9999983)
( 0.471122244, 99.9999985)
( 0.472304609, 99.9999987)
( 0.473486974, 99.9999988)
( 0.474669339, 99.999999)
( 0.475851703, 99.9999991)
( 0.477034068, 99.9999992)
( 0.478216433, 99.9999993)
( 0.479398798, 99.9999994)
( 0.480581162, 99.9999995)
( 0.481763527, 99.9999996)
( 0.482945892, 99.9999996)
( 0.484128257, 99.9999997)
( 0.485310621, 99.9999997)
( 0.486492986, 99.9999998)
( 0.487675351, 99.9999998)
( 0.488857715, 99.9999998)
( 0.49004008, 99.9999998)
( 0.491222445, 99.9999999)
( 0.49240481, 99.9999999)
( 0.493587174, 99.9999999)
( 0.494769539, 99.9999999)
( 0.495951904, 99.9999999)
( 0.497134269, 99.9999999)
( 0.498316633, 99.9999999)
( 0.499498998, 100)
( 0.500681363, 100)
( 0.501863727, 100)
( 0.503046092, 100)
( 0.504228457, 100)
( 0.505410822, 100)
( 0.506593186, 100)
( 0.507775551, 100)
( 0.508957916, 100)
( 0.510140281, 100)
( 0.511322645, 100)
( 0.51250501, 100)
( 0.513687375, 100)
( 0.514869739, 100)
( 0.516052104, 100)
( 0.517234469, 100)
( 0.518416834, 100)
( 0.519599198, 100)
( 0.520781563, 100)
( 0.521963928, 100)
( 0.523146293, 100)
( 0.524328657, 100)
( 0.525511022, 100)
( 0.526693387, 100)
( 0.527875752, 100)
( 0.529058116, 100)
( 0.530240481, 100)
( 0.531422846, 100)
( 0.53260521, 100)
( 0.533787575, 100)
( 0.53496994, 100)
( 0.536152305, 100)
( 0.537334669, 100)
( 0.538517034, 100)
( 0.539699399, 100)
( 0.540881764, 100)
( 0.542064128, 100)
( 0.543246493, 100)
( 0.544428858, 100)
( 0.545611222, 100)
( 0.546793587, 100)
( 0.547975952, 100)
( 0.549158317, 100)
( 0.550340681, 100)
( 0.551523046, 100)
( 0.552705411, 100)
( 0.553887776, 100)
( 0.55507014, 100)
( 0.556252505, 100)
( 0.55743487, 100)
( 0.558617234, 100)
( 0.559799599, 100)
( 0.560981964, 100)
( 0.562164329, 100)
( 0.563346693, 100)
( 0.564529058, 100)
( 0.565711423, 100)
( 0.566893788, 100)
( 0.568076152, 100)
( 0.569258517, 100)
( 0.570440882, 100)
( 0.571623246, 100)
( 0.572805611, 100)
( 0.573987976, 100)
( 0.575170341, 100)
( 0.576352705, 100)
( 0.57753507, 100)
( 0.578717435, 100)
( 0.5798998, 100)
( 0.581082164, 100)
( 0.582264529, 100)
( 0.583446894, 100)
( 0.584629259, 100)
( 0.585811623, 100)
( 0.586993988, 100)
( 0.588176353, 100)
( 0.589358717, 100)
( 0.590541082, 100)
( 0.591723447, 100)
( 0.592905812, 100)
( 0.594088176, 100)
( 0.595270541, 100)
( 0.596452906, 100)
( 0.597635271, 100)
( 0.598817635, 100)
( 0.6, 100)
};
\draw (axis cs:  0.4, 2.6) node {$D$};
\draw (axis cs:  0.24, 20) node {1st};
\draw (axis cs:  0.08, 40) node {2nd};
\end{semilogyaxis}


==> Gnpstrong.tex <==
\begin{axis}[
xmin= 0, xmax= 0.5,
xlabel={$p$},
ylabel={$P$(strong)},
ylabel near ticks,
]
\addplot [black,]
coordinates {
( 0.05, 0)
( 0.06122449, 0)
( 0.07244898, 0)
( 0.083673469, 0)
( 0.094897959, 0)
( 0.10612245, 0)
( 0.11734694, 0)
( 0.12857143, 0)
( 0.13979592, 0)
( 0.15102041, 0)
( 0.1622449, 0)
( 0.17346939, 0)
( 0.18469388, 0)
( 0.19591837, 0)
( 0.20714286, 0)
( 0.21836735, 0)
( 0.22959184, 0)
( 0.24081633, 0)
( 0.25204082, 0)
( 0.26326531, 0)
( 0.2744898, 0)
( 0.28571429, 0)
( 0.29693878, 0)
( 0.30816327, 0)
( 0.31938776, 0)
( 0.33061224, 0)
( 0.34183673, 0)
( 0.35306122, 0.000625)
( 0.36428571, 0)
( 0.3755102, 0.0025)
( 0.38673469, 0.006875)
( 0.39795918, 0.024375)
( 0.40918367, 0.040625)
( 0.42040816, 0.061875)
( 0.43163265, 0.13125)
( 0.44285714, 0.210625)
( 0.45408163, 0.289375)
( 0.46530612, 0.409375)
( 0.47653061, 0.50125)
( 0.4877551, 0.6125)
( 0.49897959, 0.693125)
( 0.51020408, 0.775625)
( 0.52142857, 0.860625)
( 0.53265306, 0.908125)
( 0.54387755, 0.925)
( 0.55510204, 0.96375)
( 0.56632653, 0.981875)
( 0.57755102, 0.98125)
( 0.58877551, 0.9875)
( 0.6, 0.99375)
( 0.7, 1)
( 0.9, 1)
( 0.99, 1)
};
\addplot [black,dotted]
coordinates {
( 0.01, 0.319881879)
( 0.0111823647, 0.247744327)
( 0.0123647295, 0.188086459)
( 0.0135470942, 0.140153175)
( 0.0147294589, 0.102624983)
( 0.0159118236, 0.0739240926)
( 0.0170941884, 0.052438182)
( 0.0182765531, 0.0366652523)
( 0.0194589178, 0.0252928076)
( 0.0206412826, 0.0172282015)
( 0.0218236473, 0.0115964721)
( 0.023006012, 0.00771927228)
( 0.0241883768, 0.00508502847)
( 0.0253707415, 0.00331711791)
( 0.0265531062, 0.00214410485)
( 0.0277354709, 0.00137404229)
( 0.0289178357, 0.000873493802)
( 0.0301002004, 0.000551122464)
( 0.0312825651, 0.000345282788)
( 0.0324649299, 0.00021490083)
( 0.0336472946, 0.000132930293)
( 0.0348296593, 8.17538285e-5)
( 0.036012024, 5.00098863e-5)
( 0.0371943888, 3.04384816e-5)
( 0.0383767535, 1.84397934e-5)
( 0.0395591182, 1.11222597e-5)
( 0.040741483, 6.68134215e-6)
( 0.0419238477, 3.99843577e-6)
( 0.0431062124, 2.38444304e-6)
( 0.0442885772, 1.41730043e-6)
( 0.0454709419, 8.39877882e-7)
( 0.0466533066, 4.96300252e-7)
( 0.0478356713, 2.92506768e-7)
( 0.0490180361, 1.7197834e-7)
( 0.0502004008, 1.00887193e-7)
( 0.0513827655, 5.90603221e-8)
( 0.0525651303, 3.45081261e-8)
( 0.053747495, 2.01268861e-8)
( 0.0549298597, 1.17198248e-8)
( 0.0561122244, 6.81413439e-9)
( 0.0572945892, 3.95637418e-9)
( 0.0584769539, 2.2941917e-9)
( 0.0596593186, 1.32878005e-9)
( 0.0608416834, 7.68793879e-10)
( 0.0620240481, 4.44364899e-10)
( 0.0632064128, 2.56613561e-10)
( 0.0643887776, 1.48068996e-10)
( 0.0655711423, 8.5374032e-11)
( 0.066753507, 4.91920659e-11)
( 0.0679358717, 2.83270012e-11)
( 0.0691182365, 1.63030717e-11)
( 0.0703006012, 9.37836496e-12)
( 0.0714829659, 5.39259645e-12)
( 0.0726653307, 3.09959468e-12)
( 0.0738476954, 1.78102562e-12)
( 0.0750300601, 1.02309254e-12)
( 0.0762124248, 5.8757003e-13)
( 0.0773947896, 3.37383774e-13)
( 0.0785771543, 1.93699264e-13)
( 0.079759519, 1.11196209e-13)
( 0.0809418838, 6.38306068e-14)
( 0.0821242485, 3.664068e-14)
( 0.0833066132, 2.10335295e-14)
( 0.084488978, 1.20751743e-14)
( 0.0856713427, 6.9330755e-15)
( 0.0868537074, 3.98133352e-15)
( 0.0880360721, 2.28675902e-15)
( 0.0892184369, 1.31377466e-15)
( 0.0904008016, 7.55005002e-16)
( 0.0915831663, 4.34037769e-16)
( 0.0927655311, 2.4961734e-16)
( 0.0939478958, 1.43619318e-16)
( 0.0951302605, 8.26730205e-17)
( 0.0963126253, 4.76157008e-17)
( 0.09749499, 2.74407055e-17)
( 0.0986773547, 1.58242481e-17)
( 0.0998597194, 9.13184159e-18)
( 0.101042084, 5.27383652e-18)
( 0.102224449, 3.04827613e-18)
( 0.103406814, 1.76347156e-18)
( 0.104589178, 1.02116787e-18)
( 0.105771543, 5.91928459e-19)
( 0.106953908, 3.43490284e-19)
( 0.108136273, 1.99555403e-19)
( 0.109318637, 1.16077453e-19)
( 0.110501002, 6.7608305e-20)
( 0.111683367, 3.94324165e-20)
( 0.112865731, 2.30325591e-20)
( 0.114048096, 1.3474159e-20)
( 0.115230461, 7.89528742e-21)
( 0.116412826, 4.6342354e-21)
( 0.11759519, 2.72502245e-21)
( 0.118777555, 1.60539842e-21)
( 0.11995992, 9.47667841e-22)
( 0.121142285, 5.60571153e-22)
( 0.122324649, 3.32313713e-22)
( 0.123507014, 1.97447307e-22)
( 0.124689379, 1.17593413e-22)
( 0.125871743, 7.02082076e-23)
( 0.127054108, 4.20253182e-23)
( 0.128236473, 2.52230935e-23)
( 0.129418838, 1.51808718e-23)
( 0.130601202, 9.16333837e-24)
( 0.131783567, 5.54776181e-24)
( 0.132965932, 3.36928824e-24)
( 0.134148297, 2.05288569e-24)
( 0.135330661, 1.25501326e-24)
( 0.136513026, 7.69910483e-25)
( 0.137695391, 4.74015608e-25)
( 0.138877756, 2.92926278e-25)
( 0.14006012, 1.81714985e-25)
( 0.141242485, 1.13173286e-25)
( 0.14242485, 7.07738028e-26)
( 0.143607214, 4.44459064e-26)
( 0.144789579, 2.80335034e-26)
( 0.145971944, 1.77609256e-26)
( 0.147154309, 1.13045463e-26)
( 0.148336673, 7.22931486e-27)
( 0.149519038, 4.64574261e-27)
( 0.150701403, 3.00044073e-27)
( 0.151883768, 1.94780326e-27)
( 0.153066132, 1.27114111e-27)
( 0.154248497, 8.34045683e-28)
( 0.155430862, 5.50290823e-28)
( 0.156613226, 3.6514065e-28)
( 0.157795591, 2.43698485e-28)
( 0.158977956, 1.63617413e-28)
( 0.160160321, 1.10522225e-28)
( 0.161342685, 7.51229201e-29)
( 0.16252505, 5.13874803e-29)
( 0.163707415, 3.53804522e-29)
( 0.16488978, 2.45216474e-29)
( 0.166072144, 1.71109817e-29)
( 0.167254509, 1.20225832e-29)
( 0.168436874, 8.50700106e-30)
( 0.169619238, 6.06273966e-30)
( 0.170801603, 4.35243795e-30)
( 0.171983968, 3.14792617e-30)
( 0.173166333, 2.29404171e-30)
( 0.174348697, 1.68468569e-30)
( 0.175531062, 1.24690295e-30)
( 0.176713427, 9.30244951e-31)
( 0.177895792, 6.99627564e-31)
( 0.179078156, 5.30511346e-31)
( 0.180260521, 4.05632797e-31)
( 0.181442886, 3.12776169e-31)
( 0.182625251, 2.43246802e-31)
( 0.183807615, 1.90819712e-31)
( 0.18498998, 1.51011725e-31)
( 0.186172345, 1.20574955e-31)
( 0.187354709, 9.71424672e-32)
( 0.188537074, 7.89790968e-32)
( 0.189719439, 6.48052896e-32)
( 0.190901804, 5.36719069e-32)
( 0.192084168, 4.487078e-32)
( 0.193266533, 3.78704679e-32)
( 0.194448898, 3.22698736e-32)
( 0.195631263, 2.77645792e-32)
( 0.196813627, 2.41222845e-32)
( 0.197995992, 2.11647961e-32)
( 0.199178357, 1.8754754e-32)
( 0.200360721, 1.67858012e-32)
( 0.201543086, 1.51752699e-32)
( 0.202725451, 1.38587183e-32)
( 0.203907816, 1.27858331e-32)
( 0.20509018, 1.19173503e-32)
( 0.206272545, 1.12227379e-32)
( 0.20745491, 1.06784546e-32)
( 0.208637275, 1.02666511e-32)
( 0.209819639, 9.97421221e-33)
( 0.211002004, 9.7920736e-33)
( 0.212184369, 9.71476028e-33)
( 0.213366733, 9.74011705e-33)
( 0.214549098, 9.86921145e-33)
( 0.215731463, 1.01064036e-32)
( 0.216913828, 1.04595892e-32)
( 0.218096192, 1.09406344e-32)
( 0.219278557, 1.1566035e-32)
( 0.220460922, 1.23578531e-32)
( 0.221643287, 1.33450015e-32)
( 0.222825651, 1.45649837e-32)
( 0.224008016, 1.60662307e-32)
( 0.225190381, 1.79112377e-32)
( 0.226372745, 2.01807788e-32)
( 0.22755511, 2.29795875e-32)
( 0.228737475, 2.64440466e-32)
( 0.22991984, 3.07526476e-32)
( 0.231102204, 3.61402948e-32)
( 0.232284569, 4.2917979e-32)
( 0.233466934, 5.14999946e-32)
( 0.234649299, 6.24418198e-32)
( 0.235831663, 7.64931628e-32)
( 0.237014028, 9.46727055e-32)
( 0.238196393, 1.18374082e-31)
( 0.239378758, 1.49517098e-31)
( 0.240561122, 1.90764864e-31)
( 0.241743487, 2.45837591e-31)
( 0.242925852, 3.19968946e-31)
( 0.244108216, 4.20574037e-31)
( 0.245290581, 5.5823342e-31)
( 0.246472946, 7.48151957e-31)
( 0.247655311, 1.01233555e-30)
( 0.248837675, 1.38285985e-30)
( 0.25002004, 1.90680988e-30)
( 0.251202405, 2.65379255e-30)
( 0.25238477, 3.72743397e-30)
( 0.253567134, 5.28308616e-30)
( 0.254749499, 7.55526664e-30)
( 0.255931864, 1.09004441e-29)
( 0.257114228, 1.58641614e-29)
( 0.258296593, 2.32869793e-29)
( 0.259478958, 3.44726939e-29)
( 0.260661323, 5.14570174e-29)
( 0.261843687, 7.74392244e-29)
( 0.263026052, 1.174796e-28)
( 0.264208417, 1.79632751e-28)
( 0.265390782, 2.76799395e-28)
( 0.266573146, 4.29768666e-28)
( 0.267755511, 6.72243007e-28)
( 0.268937876, 1.05918114e-27)
( 0.27012024, 1.68072091e-27)
( 0.271302605, 2.68552995e-27)
( 0.27248497, 4.3201582e-27)
( 0.273667335, 6.99567188e-27)
( 0.274849699, 1.14009989e-26)
( 0.276032064, 1.86965879e-26)
( 0.277214429, 3.08467083e-26)
( 0.278396794, 5.11920079e-26)
( 0.279579158, 8.54399643e-26)
( 0.280761523, 1.4338479e-25)
( 0.281943888, 2.41904947e-25)
( 0.283126253, 4.10205562e-25)
( 0.284308617, 6.99017402e-25)
( 0.285490982, 1.19678924e-24)
( 0.286673347, 2.05827474e-24)
( 0.287855711, 3.55514169e-24)
( 0.289038076, 6.16580167e-24)
( 0.290220441, 1.07352392e-23)
( 0.291402806, 1.87600187e-23)
( 0.29258517, 3.2897541e-23)
( 0.293767535, 5.78776619e-23)
( 0.2949499, 1.02137256e-22)
( 0.296132265, 1.80755275e-22)
( 0.297314629, 3.20729533e-22)
( 0.298496994, 5.70473478e-22)
( 0.299679359, 1.01692207e-21)
( 0.300861723, 1.81636306e-21)
( 0.302044088, 3.25003065e-21)
( 0.303226453, 5.82437226e-21)
( 0.304408818, 1.04518903e-20)
( 0.305591182, 1.87772491e-20)
( 0.306773547, 3.37651056e-20)
( 0.307955912, 6.07590843e-20)
( 0.309138277, 1.09387989e-19)
( 0.310320641, 1.96993631e-19)
( 0.311503006, 3.5478744e-19)
( 0.312685371, 6.38892503e-19)
( 0.313867735, 1.15011573e-18)
( 0.3150501, 2.06928809e-18)
( 0.316232465, 3.72030321e-18)
( 0.31741483, 6.68231432e-18)
( 0.318597194, 1.19889416e-17)
( 0.319779559, 2.14810457e-17)
( 0.320961924, 3.84296995e-17)
( 0.322144289, 6.86330185e-17)
( 0.323326653, 1.22341147e-16)
( 0.324509018, 2.17623322e-16)
( 0.325691383, 3.86236431e-16)
( 0.326873747, 6.83815355e-16)
( 0.328056112, 1.20749867e-15)
( 0.329238477, 2.12629048e-15)
( 0.330420842, 3.73313906e-15)
( 0.331603206, 6.53387065e-15)
( 0.332785571, 1.13983643e-14)
( 0.333967936, 1.98163081e-14)
( 0.335150301, 3.43277641e-14)
( 0.336332665, 5.92443598e-14)
( 0.33751503, 1.01850986e-13)
( 0.338697395, 1.74397436e-13)
( 0.33987976, 2.9738112e-13)
( 0.341062124, 5.04927336e-13)
( 0.342244489, 8.53556524e-13)
( 0.343426854, 1.43638649e-12)
( 0.344609218, 2.40600032e-12)
( 0.345791583, 4.01104133e-12)
( 0.346973948, 6.6544086e-12)
( 0.348156313, 1.09852133e-11)
( 0.349338677, 1.80431402e-11)
( 0.350521042, 2.94835855e-11)
( 0.351703407, 4.79264254e-11)
( 0.352885772, 7.74926341e-11)
( 0.354068136, 1.24624261e-10)
( 0.355250501, 1.99328661e-10)
( 0.356432866, 3.17053188e-10)
( 0.35761523, 5.01489674e-10)
( 0.358797595, 7.88739616e-10)
( 0.35997996, 1.23345527e-9)
( 0.361162325, 1.91782744e-9)
( 0.362344689, 2.96464214e-9)
( 0.363527054, 4.55610627e-9)
( 0.364709419, 6.960787e-9)
( 0.365891784, 1.05718691e-8)
( 0.367074148, 1.59610704e-8)
( 0.368256513, 2.39540388e-8)
( 0.369438878, 3.57349753e-8)
( 0.370621242, 5.29906799e-8)
( 0.371803607, 7.81073256e-8)
( 0.372985972, 1.14437144e-7)
( 0.374168337, 1.66657006e-7)
( 0.375350701, 2.41246732e-7)
( 0.376533066, 3.47122016e-7)
( 0.377715431, 4.96465225e-7)
( 0.378897796, 7.05807157e-7)
( 0.38008016, 9.97424161e-7)
( 0.381262525, 1.40112789e-6)
( 0.38244489, 1.95653931e-6)
( 0.383627255, 2.71595423e-6)
( 0.384809619, 3.74792446e-6)
( 0.385991984, 5.14169615e-6)
( 0.387174349, 7.01266449e-6)
( 0.388356713, 9.50902112e-6)
( 0.389539078, 1.28197864e-5)
( 0.390721443, 1.71844318e-5)
( 0.391903808, 2.29043082e-5)
( 0.393086172, 3.03560992e-5)
( 0.394268537, 4.00075193e-5)
( 0.395450902, 5.24354664e-5)
( 0.396633267, 6.83468197e-5)
( 0.397815631, 8.8602047e-5)
( 0.398997996, 0.000114241745)
( 0.400180361, 0.000146516183)
( 0.401362725, 0.000186917855)
( 0.40254509, 0.000237216977)
( 0.403727455, 0.00029949976)
( 0.40490982, 0.000376209202)
( 0.406092184, 0.000470188031)
( 0.407274549, 0.000584723319)
( 0.408456914, 0.000723592148)
( 0.409639279, 0.000891107617)
( 0.410821643, 0.00109216435)
( 0.412004008, 0.00133228257)
( 0.413186373, 0.00161764964)
( 0.414368737, 0.00195515809)
( 0.415551102, 0.0023524388)
( 0.416733467, 0.00281788825)
( 0.417915832, 0.00336068865)
( 0.419098196, 0.00399081969)
( 0.420280561, 0.00471906094)
( 0.421462926, 0.00555698382)
( 0.422645291, 0.00651693233)
( 0.423827655, 0.00761199179)
( 0.42501002, 0.00885594518)
( 0.426192385, 0.0102632167)
( 0.427374749, 0.0118488026)
( 0.428557114, 0.0136281895)
( 0.429739479, 0.0156172602)
( 0.430921844, 0.0178321889)
( 0.432104208, 0.0202893251)
( 0.433286573, 0.0230050693)
( 0.434468938, 0.02599574)
( 0.435651303, 0.0292774349)
( 0.436833667, 0.0328658882)
( 0.438016032, 0.0367763249)
( 0.439198397, 0.0410233149)
( 0.440380762, 0.0456206283)
( 0.441563126, 0.0505810947)
( 0.442745491, 0.0559164683)
( 0.443927856, 0.0616372997)
( 0.44511022, 0.0677528176)
( 0.446292585, 0.0742708214)
( 0.44747495, 0.0811975858)
( 0.448657315, 0.0885377794)
( 0.449839679, 0.0962943979)
( 0.451022044, 0.104468712)
( 0.452204409, 0.113060234)
( 0.453386774, 0.122066694)
( 0.454569138, 0.131484042)
( 0.455751503, 0.141306458)
( 0.456933868, 0.151526381)
( 0.458116232, 0.162134553)
( 0.459298597, 0.173120077)
( 0.460480962, 0.184470488)
( 0.461663327, 0.196171833)
( 0.462845691, 0.208208769)
( 0.464028056, 0.220564665)
( 0.465210421, 0.23322171)
( 0.466392786, 0.246161034)
( 0.46757515, 0.259362829)
( 0.468757515, 0.272806477)
( 0.46993988, 0.286470674)
( 0.471122244, 0.300333567)
( 0.472304609, 0.314372875)
( 0.473486974, 0.328566022)
( 0.474669339, 0.34289026)
( 0.475851703, 0.357322787)
( 0.477034068, 0.371840867)
( 0.478216433, 0.38642194)
( 0.479398798, 0.401043724)
( 0.480581162, 0.415684313)
( 0.481763527, 0.430322272)
( 0.482945892, 0.444936714)
( 0.484128257, 0.45950738)
( 0.485310621, 0.474014702)
( 0.486492986, 0.488439868)
( 0.487675351, 0.502764867)
( 0.488857715, 0.516972538)
( 0.49004008, 0.531046605)
( 0.491222445, 0.544971703)
( 0.49240481, 0.558733404)
( 0.493587174, 0.572318229)
( 0.494769539, 0.585713658)
( 0.495951904, 0.598908132)
( 0.497134269, 0.61189105)
( 0.498316633, 0.624652765)
( 0.499498998, 0.637184563)
( 0.500681363, 0.649478657)
( 0.501863727, 0.661528159)
( 0.503046092, 0.673327057)
( 0.504228457, 0.684870192)
( 0.505410822, 0.696153225)
( 0.506593186, 0.707172609)
( 0.507775551, 0.717925554)
( 0.508957916, 0.72840999)
( 0.510140281, 0.738624539)
( 0.511322645, 0.748568472)
( 0.51250501, 0.758241675)
( 0.513687375, 0.767644611)
( 0.514869739, 0.776778286)
( 0.516052104, 0.785644209)
( 0.517234469, 0.79424436)
( 0.518416834, 0.802581149)
( 0.519599198, 0.810657386)
( 0.520781563, 0.818476246)
( 0.521963928, 0.826041235)
( 0.523146293, 0.83335616)
( 0.524328657, 0.840425096)
( 0.525511022, 0.84725236)
( 0.526693387, 0.85384248)
( 0.527875752, 0.860200171)
( 0.529058116, 0.866330305)
( 0.530240481, 0.872237895)
( 0.531422846, 0.877928062)
( 0.53260521, 0.883406022)
( 0.533787575, 0.888677063)
( 0.53496994, 0.893746525)
( 0.536152305, 0.898619785)
( 0.537334669, 0.903302237)
( 0.538517034, 0.907799282)
( 0.539699399, 0.91211631)
( 0.540881764, 0.916258689)
( 0.542064128, 0.920231754)
( 0.543246493, 0.924040794)
( 0.544428858, 0.927691044)
( 0.545611222, 0.931187676)
( 0.546793587, 0.934535794)
( 0.547975952, 0.937740419)
( 0.549158317, 0.940806492)
( 0.550340681, 0.943738864)
( 0.551523046, 0.946542292)
( 0.552705411, 0.949221432)
( 0.553887776, 0.951780842)
( 0.55507014, 0.954224974)
( 0.556252505, 0.956558174)
( 0.55743487, 0.958784678)
( 0.558617234, 0.960908613)
( 0.559799599, 0.962933994)
( 0.560981964, 0.964864726)
( 0.562164329, 0.966704601)
( 0.563346693, 0.968457301)
( 0.564529058, 0.970126393)
( 0.565711423, 0.971715338)
( 0.566893788, 0.973227485)
( 0.568076152, 0.974666075)
( 0.569258517, 0.976034241)
( 0.570440882, 0.977335011)
( 0.571623246, 0.97857131)
( 0.572805611, 0.979745959)
( 0.573987976, 0.98086168)
( 0.575170341, 0.981921096)
( 0.576352705, 0.982926734)
( 0.57753507, 0.983881028)
( 0.578717435, 0.984786318)
( 0.5798998, 0.985644856)
( 0.581082164, 0.986458807)
( 0.582264529, 0.98723025)
( 0.583446894, 0.987961182)
( 0.584629259, 0.98865352)
( 0.585811623, 0.989309103)
( 0.586993988, 0.989929694)
( 0.588176353, 0.990516983)
( 0.589358717, 0.99107259)
( 0.590541082, 0.991598066)
( 0.591723447, 0.992094895)
( 0.592905812, 0.992564498)
( 0.594088176, 0.993008233)
( 0.595270541, 0.993427398)
( 0.596452906, 0.993823237)
( 0.597635271, 0.994196933)
( 0.598817635, 0.99454962)
( 0.6, 0.994882379)
};
\addplot [red  ,dashed]
coordinates {
( 0.03, 0)
( 0.03755102, 0)
( 0.045102041, 0)
( 0.052653061, 0)
( 0.060204082, 0)
( 0.067755102, 0)
( 0.075306122, 0)
( 0.082857143, 0)
( 0.090408163, 0)
( 0.097959184, 0)
( 0.1055102, 0)
( 0.11306122, 0)
( 0.12061224, 0)
( 0.12816327, 0)
( 0.13571429, 0)
( 0.14326531, 0)
( 0.15081633, 0)
( 0.15836735, 0)
( 0.16591837, 0)
( 0.17346939, 0)
( 0.18102041, 0)
( 0.18857143, 0)
( 0.19612245, 0)
( 0.20367347, 0)
( 0.21122449, 0)
( 0.21877551, 0)
( 0.22632653, 0)
( 0.23387755, 0)
( 0.24142857, 0)
( 0.24897959, 0)
( 0.25653061, 0)
( 0.26408163, 0)
( 0.27163265, 0)
( 0.27918367, 0.0025)
( 0.28673469, 0.01)
( 0.29428571, 0.055)
( 0.30183673, 0.1025)
( 0.30938776, 0.24)
( 0.31693878, 0.365)
( 0.3244898, 0.5325)
( 0.33204082, 0.6925)
( 0.33959184, 0.7875)
( 0.34714286, 0.89)
( 0.35469388, 0.92)
( 0.3622449, 0.9725)
( 0.36979592, 0.975)
( 0.37734694, 0.98)
( 0.38489796, 0.9925)
( 0.39244898, 0.9925)
( 0.4, 0.9925)
( 0.6, 1)
( 0.8, 1)
( 0.99, 1)
};
\addplot [red  ,dotted]
coordinates {
( 0.01, 3.32449311e-13)
( 0.0111823647, 1.2339845e-15)
( 0.0123647295, 3.55830454e-18)
( 0.0135470942, 8.25082137e-21)
( 0.0147294589, 1.58467841e-23)
( 0.0159118236, 2.58643811e-26)
( 0.0170941884, 3.66813469e-29)
( 0.0182765531, 4.60887966e-32)
( 0.0194589178, 5.21811639e-35)
( 0.0206412826, 5.40309619e-38)
( 0.0218236473, 5.18351376e-41)
( 0.023006012, 4.66015157e-44)
( 0.0241883768, 3.96548265e-47)
( 0.0253707415, 3.22178045e-50)
( 0.0265531062, 2.51828668e-53)
( 0.0277354709, 1.90637306e-56)
( 0.0289178357, 1.40578189e-59)
( 0.0301002004, 1.0149038e-62)
( 0.0312825651, 7.20503113e-66)
( 0.0324649299, 5.04909953e-69)
( 0.0336472946, 3.50439426e-72)
( 0.0348296593, 2.41607076e-75)
( 0.036012024, 1.65894781e-78)
( 0.0371943888, 1.13707598e-81)
( 0.0383767535, 7.796323e-85)
( 0.0395591182, 5.35756975e-88)
( 0.040741483, 3.6965883e-91)
( 0.0419238477, 2.56523816e-94)
( 0.0431062124, 1.79333438e-97)
( 0.0442885772, 1.26503908e-100)
( 0.0454709419, 9.01897986e-104)
( 0.0466533066, 6.5092726e-107)
( 0.0478356713, 4.76383516e-110)
( 0.0490180361, 3.54145075e-113)
( 0.0502004008, 2.67907835e-116)
( 0.0513827655, 2.06624326e-119)
( 0.0525651303, 1.62786018e-122)
( 0.053747495, 1.31273812e-125)
( 0.0549298597, 1.08589959e-128)
( 0.0561122244, 9.23458728e-132)
( 0.0572945892, 8.09222844e-135)
( 0.0584769539, 7.3246874e-138)
( 0.0596593186, 6.86544172e-141)
( 0.0608416834, 6.68089173e-144)
( 0.0620240481, 6.76790499e-147)
( 0.0632064128, 7.15703919e-150)
( 0.0643887776, 7.92344833e-153)
( 0.0655711423, 9.21031893e-156)
( 0.066753507, 1.12752617e-158)
( 0.0679358717, 1.45819089e-161)
( 0.0691182365, 1.99853935e-164)
( 0.0703006012, 2.9122254e-167)
( 0.0714829659, 4.52669387e-170)
( 0.0726653307, 7.53069988e-173)
( 0.0738476954, 1.34543846e-175)
( 0.0750300601, 2.59037338e-178)
( 0.0762124248, 5.3931647e-181)
( 0.0773947896, 1.21852617e-183)
( 0.0785771543, 2.99829654e-186)
( 0.079759519, 8.0632532e-189)
( 0.0809418838, 2.37845732e-191)
( 0.0821242485, 7.72300155e-194)
( 0.0833066132, 2.77037766e-196)
( 0.084488978, 1.10181189e-198)
( 0.0856713427, 4.87572607e-201)
( 0.0868537074, 2.40920417e-203)
( 0.0880360721, 1.33394534e-205)
( 0.0892184369, 8.30512347e-208)
( 0.0904008016, 5.83437783e-210)
( 0.0915831663, 4.64045925e-212)
( 0.0927655311, 4.19277313e-214)
( 0.0939478958, 4.31765663e-216)
( 0.0951302605, 5.0840273e-218)
( 0.0963126253, 6.86688754e-220)
( 0.09749499, 1.06722135e-221)
( 0.0986773547, 1.9143061e-223)
( 0.0998597194, 3.97483184e-225)
( 0.101042084, 9.58147178e-227)
( 0.102224449, 2.68889582e-228)
( 0.103406814, 8.80911348e-230)
( 0.104589178, 3.37800782e-231)
( 0.105771543, 1.52012155e-232)
( 0.106953908, 8.04765414e-234)
( 0.108136273, 5.02438357e-235)
( 0.109318637, 3.70794293e-236)
( 0.110501002, 3.24189961e-237)
( 0.111683367, 3.36532654e-238)
( 0.112865731, 4.15648646e-239)
( 0.114048096, 6.12030528e-240)
( 0.115230461, 1.07648792e-240)
( 0.116412826, 2.26590754e-241)
( 0.11759519, 5.71801727e-242)
( 0.118777555, 1.73283751e-242)
( 0.11995992, 6.31659988e-243)
( 0.121142285, 2.77390024e-243)
( 0.122324649, 1.46964731e-243)
( 0.123507014, 9.40689634e-244)
( 0.124689379, 7.28364701e-244)
( 0.125871743, 6.83030455e-244)
( 0.127054108, 7.76602525e-244)
( 0.128236473, 1.07167204e-243)
( 0.129418838, 1.79647951e-243)
( 0.130601202, 3.66122834e-243)
( 0.131783567, 9.07766677e-243)
( 0.132965932, 2.73976045e-242)
( 0.134148297, 1.00701679e-241)
( 0.135330661, 4.50905405e-241)
( 0.136513026, 2.46002078e-240)
( 0.137695391, 1.6353655e-239)
( 0.138877756, 1.32454513e-238)
( 0.14006012, 1.30671098e-237)
( 0.141242485, 1.56951967e-236)
( 0.14242485, 2.29386223e-235)
( 0.143607214, 4.07607527e-234)
( 0.144789579, 8.79773916e-233)
( 0.145971944, 2.30382384e-231)
( 0.147154309, 7.30944554e-230)
( 0.148336673, 2.80539229e-228)
( 0.149519038, 1.30017014e-226)
( 0.150701403, 7.26158207e-225)
( 0.151883768, 4.87657428e-223)
( 0.153066132, 3.92805567e-221)
( 0.154248497, 3.78479808e-219)
( 0.155430862, 4.34938338e-217)
( 0.156613226, 5.94214218e-215)
( 0.157795591, 9.618133e-213)
( 0.158977956, 1.83765284e-210)
( 0.160160321, 4.128037e-208)
( 0.161342685, 1.08568344e-205)
( 0.16252505, 3.32816039e-203)
( 0.163707415, 1.18358348e-200)
( 0.16488978, 4.85881874e-198)
( 0.166072144, 2.29052998e-195)
( 0.167254509, 1.23323479e-192)
( 0.168436874, 7.54029266e-190)
( 0.169619238, 5.20464879e-187)
( 0.170801603, 4.03076056e-184)
( 0.171983968, 3.48027673e-181)
( 0.173166333, 3.32829899e-178)
( 0.174348697, 3.50170742e-175)
( 0.175531062, 4.02508966e-172)
( 0.176713427, 5.0191081e-169)
( 0.177895792, 6.7403771e-166)
( 0.179078156, 9.67700388e-163)
( 0.180260521, 1.47413553e-159)
( 0.181442886, 2.36466872e-156)
( 0.182625251, 3.96369387e-153)
( 0.183807615, 6.88905343e-150)
( 0.18498998, 1.23186249e-146)
( 0.186172345, 2.24859591e-143)
( 0.187354709, 4.15727884e-140)
( 0.188537074, 7.72441243e-137)
( 0.189719439, 1.43122396e-133)
( 0.190901804, 2.62415503e-130)
( 0.192084168, 4.7249909e-127)
( 0.193266533, 8.29234022e-124)
( 0.194448898, 1.40801495e-120)
( 0.195631263, 2.2963816e-117)
( 0.196813627, 3.57200478e-114)
( 0.197995992, 5.26278983e-111)
( 0.199178357, 7.29540133e-108)
( 0.200360721, 9.45367277e-105)
( 0.201543086, 1.13805236e-101)
( 0.202725451, 1.26513243e-98)
( 0.203907816, 1.29133615e-95)
( 0.20509018, 1.20367986e-92)
( 0.206272545, 1.01933278e-89)
( 0.20745491, 7.80458244e-87)
( 0.208637275, 5.37825584e-84)
( 0.209819639, 3.32167971e-81)
( 0.211002004, 1.83148869e-78)
( 0.212184369, 8.98312567e-76)
( 0.213366733, 3.90675193e-73)
( 0.214549098, 1.50210333e-70)
( 0.215731463, 5.09274172e-68)
( 0.216913828, 1.51909315e-65)
( 0.218096192, 3.978784e-63)
( 0.219278557, 9.13563907e-61)
( 0.220460922, 1.83642844e-58)
( 0.221643287, 3.22857463e-56)
( 0.222825651, 4.96057921e-54)
( 0.224008016, 6.65802536e-52)
( 0.225190381, 7.80505836e-50)
( 0.226372745, 7.99218231e-48)
( 0.22755511, 7.15094981e-46)
( 0.228737475, 5.59404985e-44)
( 0.22991984, 3.82919474e-42)
( 0.231102204, 2.29591039e-40)
( 0.232284569, 1.20727032e-38)
( 0.233466934, 5.57537587e-37)
( 0.234649299, 2.26494753e-35)
( 0.235831663, 8.10814425e-34)
( 0.237014028, 2.56267754e-32)
( 0.238196393, 7.16580027e-31)
( 0.239378758, 1.77654561e-29)
( 0.240561122, 3.91399074e-28)
( 0.241743487, 7.68119248e-27)
( 0.242925852, 1.34609037e-25)
( 0.244108216, 2.11183714e-24)
( 0.245290581, 2.97384955e-23)
( 0.246472946, 3.76881523e-22)
( 0.247655311, 4.310143e-21)
( 0.248837675, 4.46033798e-20)
( 0.25002004, 4.18824422e-19)
( 0.251202405, 3.57841011e-18)
( 0.25238477, 2.78965946e-17)
( 0.253567134, 1.98986839e-16)
( 0.254749499, 1.30231393e-15)
( 0.255931864, 7.84197399e-15)
( 0.257114228, 4.35657484e-14)
( 0.258296593, 2.23900879e-13)
( 0.259478958, 1.06739431e-12)
( 0.260661323, 4.73265568e-12)
( 0.261843687, 1.95673224e-11)
( 0.263026052, 7.56347346e-11)
( 0.264208417, 2.74013186e-10)
( 0.265390782, 9.32733349e-10)
( 0.266573146, 2.99042257e-9)
( 0.267755511, 9.05162151e-9)
( 0.268937876, 2.59265374e-8)
( 0.27012024, 7.04316083e-8)
( 0.271302605, 1.81865721e-7)
( 0.27248497, 4.47325405e-7)
( 0.273667335, 1.05024076e-6)
( 0.274849699, 2.35843251e-6)
( 0.276032064, 5.07548397e-6)
( 0.277214429, 1.04875598e-5)
( 0.278396794, 2.08454582e-5)
( 0.279579158, 3.99262983e-5)
( 0.280761523, 7.38178893e-5)
( 0.281943888, 0.000131958556)
( 0.283126253, 0.000228443883)
( 0.284308617, 0.000383579091)
( 0.285490982, 0.000625613557)
( 0.286673347, 0.000992547101)
( 0.287855711, 0.00153385294)
( 0.289038076, 0.00231192788)
( 0.290220441, 0.003403064)
( 0.291402806, 0.00489774378)
( 0.29258517, 0.00690009456)
( 0.293767535, 0.00952639625)
( 0.2949499, 0.0129026136)
( 0.296132265, 0.0171610107)
( 0.297314629, 0.0224359917)
( 0.298496994, 0.0288593857)
( 0.299679359, 0.0365554486)
( 0.300861723, 0.0456358822)
( 0.302044088, 0.0561951739)
( 0.303226453, 0.0683065292)
( 0.304408818, 0.0820186269)
( 0.305591182, 0.0973533558)
( 0.306773547, 0.114304626)
( 0.307955912, 0.132838268)
( 0.309138277, 0.152892974)
( 0.310320641, 0.174382165)
( 0.311503006, 0.197196642)
( 0.312685371, 0.221207843)
( 0.313867735, 0.246271507)
( 0.3150501, 0.27223157)
( 0.316232465, 0.298924101)
( 0.31741483, 0.326181142)
( 0.318597194, 0.353834303)
( 0.319779559, 0.381718029)
( 0.320961924, 0.409672453)
( 0.322144289, 0.43754581)
( 0.323326653, 0.465196382)
( 0.324509018, 0.492493975)
( 0.325691383, 0.519320963)
( 0.326873747, 0.54557292)
( 0.328056112, 0.571158888)
( 0.329238477, 0.59600133)
( 0.330420842, 0.620035813)
( 0.331603206, 0.643210478)
( 0.332785571, 0.665485338)
( 0.333967936, 0.686831455)
( 0.335150301, 0.70723003)
( 0.336332665, 0.726671446)
( 0.33751503, 0.745154288)
( 0.338697395, 0.762684375)
( 0.33987976, 0.779273805)
( 0.341062124, 0.794940054)
( 0.342244489, 0.809705115)
( 0.343426854, 0.823594707)
( 0.344609218, 0.836637539)
( 0.345791583, 0.84886465)
( 0.346973948, 0.860308809)
( 0.348156313, 0.871003986)
( 0.349338677, 0.880984887)
( 0.350521042, 0.890286548)
( 0.351703407, 0.898943986)
( 0.352885772, 0.906991904)
( 0.354068136, 0.914464446)
( 0.355250501, 0.92139499)
( 0.356432866, 0.927815982)
( 0.35761523, 0.933758812)
( 0.358797595, 0.939253709)
( 0.35997996, 0.944329673)
( 0.361162325, 0.949014422)
( 0.362344689, 0.953334364)
( 0.363527054, 0.957314588)
( 0.364709419, 0.960978859)
( 0.365891784, 0.96434964)
( 0.367074148, 0.967448107)
( 0.368256513, 0.970294186)
( 0.369438878, 0.972906591)
( 0.370621242, 0.97530286)
( 0.371803607, 0.977499408)
( 0.372985972, 0.979511568)
( 0.374168337, 0.981353649)
( 0.375350701, 0.983038976)
( 0.376533066, 0.984579953)
( 0.377715431, 0.985988102)
( 0.378897796, 0.987274118)
( 0.38008016, 0.98844792)
( 0.381262525, 0.989518692)
( 0.38244489, 0.990494932)
( 0.383627255, 0.991384495)
( 0.384809619, 0.992194638)
( 0.385991984, 0.992932053)
( 0.387174349, 0.993602914)
( 0.388356713, 0.994212905)
( 0.389539078, 0.99476726)
( 0.390721443, 0.995270792)
( 0.391903808, 0.995727926)
( 0.393086172, 0.996142724)
( 0.394268537, 0.996518916)
( 0.395450902, 0.996859923)
( 0.396633267, 0.99716888)
( 0.397815631, 0.997448659)
( 0.398997996, 0.997701889)
( 0.400180361, 0.997930974)
( 0.401362725, 0.998138115)
( 0.40254509, 0.998325319)
( 0.403727455, 0.998494422)
( 0.40490982, 0.998647099)
( 0.406092184, 0.998784877)
( 0.407274549, 0.998909148)
( 0.408456914, 0.999021181)
( 0.409639279, 0.999122131)
( 0.410821643, 0.999213051)
( 0.412004008, 0.999294895)
( 0.413186373, 0.999368533)
( 0.414368737, 0.999434756)
( 0.415551102, 0.99949428)
( 0.416733467, 0.999547757)
( 0.417915832, 0.999595776)
( 0.419098196, 0.999638874)
( 0.420280561, 0.999677535)
( 0.421462926, 0.999712199)
( 0.422645291, 0.999743264)
( 0.423827655, 0.999771089)
( 0.42501002, 0.999796)
( 0.426192385, 0.99981829)
( 0.427374749, 0.999838226)
( 0.428557114, 0.999856046)
( 0.429739479, 0.999871968)
( 0.430921844, 0.999886186)
( 0.432104208, 0.999898876)
( 0.433286573, 0.999910197)
( 0.434468938, 0.999920291)
( 0.435651303, 0.999929287)
( 0.436833667, 0.999937299)
( 0.438016032, 0.999944432)
( 0.439198397, 0.999950779)
( 0.440380762, 0.999956423)
( 0.441563126, 0.99996144)
( 0.442745491, 0.999965897)
( 0.443927856, 0.999969855)
( 0.44511022, 0.999973367)
( 0.446292585, 0.999976483)
( 0.44747495, 0.999979245)
( 0.448657315, 0.999981692)
( 0.449839679, 0.999983859)
( 0.451022044, 0.999985777)
( 0.452204409, 0.999987474)
( 0.453386774, 0.999988975)
( 0.454569138, 0.9999903)
( 0.455751503, 0.999991471)
( 0.456933868, 0.999992505)
( 0.458116232, 0.999993417)
( 0.459298597, 0.999994221)
( 0.460480962, 0.99999493)
( 0.461663327, 0.999995554)
( 0.462845691, 0.999996104)
( 0.464028056, 0.999996587)
( 0.465210421, 0.999997012)
( 0.466392786, 0.999997386)
( 0.46757515, 0.999997714)
( 0.468757515, 0.999998002)
( 0.46993988, 0.999998255)
( 0.471122244, 0.999998476)
( 0.472304609, 0.999998671)
( 0.473486974, 0.999998841)
( 0.474669339, 0.99999899)
( 0.475851703, 0.99999912)
( 0.477034068, 0.999999234)
( 0.478216433, 0.999999334)
( 0.479398798, 0.999999421)
( 0.480581162, 0.999999496)
( 0.481763527, 0.999999563)
( 0.482945892, 0.99999962)
( 0.484128257, 0.999999671)
( 0.485310621, 0.999999715)
( 0.486492986, 0.999999753)
( 0.487675351, 0.999999786)
( 0.488857715, 0.999999815)
( 0.49004008, 0.99999984)
( 0.491222445, 0.999999861)
( 0.49240481, 0.99999988)
( 0.493587174, 0.999999897)
( 0.494769539, 0.999999911)
( 0.495951904, 0.999999923)
( 0.497134269, 0.999999934)
( 0.498316633, 0.999999943)
( 0.499498998, 0.999999951)
( 0.500681363, 0.999999958)
( 0.501863727, 0.999999964)
( 0.503046092, 0.999999969)
( 0.504228457, 0.999999973)
( 0.505410822, 0.999999977)
( 0.506593186, 0.99999998)
( 0.507775551, 0.999999983)
( 0.508957916, 0.999999986)
( 0.510140281, 0.999999988)
( 0.511322645, 0.999999989)
( 0.51250501, 0.999999991)
( 0.513687375, 0.999999992)
( 0.514869739, 0.999999993)
( 0.516052104, 0.999999994)
( 0.517234469, 0.999999995)
( 0.518416834, 0.999999996)
( 0.519599198, 0.999999997)
( 0.520781563, 0.999999997)
( 0.521963928, 0.999999997)
( 0.523146293, 0.999999998)
( 0.524328657, 0.999999998)
( 0.525511022, 0.999999998)
( 0.526693387, 0.999999999)
( 0.527875752, 0.999999999)
( 0.529058116, 0.999999999)
( 0.530240481, 0.999999999)
( 0.531422846, 0.999999999)
( 0.53260521, 0.999999999)
( 0.533787575, 1)
( 0.53496994, 1)
( 0.536152305, 1)
( 0.537334669, 1)
( 0.538517034, 1)
( 0.539699399, 1)
( 0.540881764, 1)
( 0.542064128, 1)
( 0.543246493, 1)
( 0.544428858, 1)
( 0.545611222, 1)
( 0.546793587, 1)
( 0.547975952, 1)
( 0.549158317, 1)
( 0.550340681, 1)
( 0.551523046, 1)
( 0.552705411, 1)
( 0.553887776, 1)
( 0.55507014, 1)
( 0.556252505, 1)
( 0.55743487, 1)
( 0.558617234, 1)
( 0.559799599, 1)
( 0.560981964, 1)
( 0.562164329, 1)
( 0.563346693, 1)
( 0.564529058, 1)
( 0.565711423, 1)
( 0.566893788, 1)
( 0.568076152, 1)
( 0.569258517, 1)
( 0.570440882, 1)
( 0.571623246, 1)
( 0.572805611, 1)
( 0.573987976, 1)
( 0.575170341, 1)
( 0.576352705, 1)
( 0.57753507, 1)
( 0.578717435, 1)
( 0.5798998, 1)
( 0.581082164, 1)
( 0.582264529, 1)
( 0.583446894, 1)
( 0.584629259, 1)
( 0.585811623, 1)
( 0.586993988, 1)
( 0.588176353, 1)
( 0.589358717, 1)
( 0.590541082, 1)
( 0.591723447, 1)
( 0.592905812, 1)
( 0.594088176, 1)
( 0.595270541, 1)
( 0.596452906, 1)
( 0.597635271, 1)
( 0.598817635, 1)
( 0.6, 1)
};
\addplot [gray ,]
coordinates {
( 0.019, 0)
( 0.023714286, 0)
( 0.028428571, 0)
( 0.033142857, 0)
( 0.037857143, 0)
( 0.042571429, 0)
( 0.047285714, 0)
( 0.052, 0)
( 0.056714286, 0)
( 0.061428571, 0)
( 0.066142857, 0)
( 0.070857143, 0)
( 0.075571429, 0)
( 0.080285714, 0)
( 0.085, 0)
( 0.089714286, 0)
( 0.094428571, 0)
( 0.099142857, 0)
( 0.10385714, 0)
( 0.10857143, 0)
( 0.11328571, 0)
( 0.118, 0)
( 0.12271429, 0)
( 0.12742857, 0)
( 0.13214286, 0)
( 0.13685714, 0)
( 0.14157143, 0)
( 0.14628571, 0)
( 0.151, 0)
( 0.15571429, 0)
( 0.16042857, 0)
( 0.16514286, 0)
( 0.16985714, 0)
( 0.17457143, 0)
( 0.17928571, 0)
( 0.184, 0)
( 0.18871429, 0.01)
( 0.19342857, 0.0625)
( 0.19814286, 0.19)
( 0.20285714, 0.4225)
( 0.20757143, 0.6025)
( 0.21228571, 0.69)
( 0.217, 0.835)
( 0.22171429, 0.9325)
( 0.22642857, 0.9525)
( 0.23114286, 0.9675)
( 0.23585714, 0.9925)
( 0.24057143, 0.9925)
( 0.24528571, 1)
( 0.25, 1)
( 0.3, 1)
( 0.6, 1)
( 0.99, 1)
};
\addplot [gray ,dotted]
coordinates {
( 0.01, 2.58979617e-228)
( 0.0111823647, 1.20173945e-264)
( 0.0123647295, 2.02519243e-301)
( 0.0135470942, 0)
( 0.0147294589, 0)
( 0.0159118236, 0)
( 0.0170941884, 0)
( 0.0182765531, 0)
( 0.0194589178, 0)
( 0.0206412826, 0)
( 0.0218236473, 0)
( 0.023006012, 0)
( 0.0241883768, 0)
( 0.0253707415, 0)
( 0.0265531062, 0)
( 0.0277354709, 0)
( 0.0289178357, 0)
( 0.0301002004, 0)
( 0.0312825651, 0)
( 0.0324649299, 0)
( 0.0336472946, 0)
( 0.0348296593, 0)
( 0.036012024, 0)
( 0.0371943888, 0)
( 0.0383767535, 0)
( 0.0395591182, 0)
( 0.040741483, 0)
( 0.0419238477, 0)
( 0.0431062124, 0)
( 0.0442885772, 0)
( 0.0454709419, 0)
( 0.0466533066, 0)
( 0.0478356713, 0)
( 0.0490180361, 0)
( 0.0502004008, 0)
( 0.0513827655, 0)
( 0.0525651303, 0)
( 0.053747495, 0)
( 0.0549298597, 0)
( 0.0561122244, 0)
( 0.0572945892, 0)
( 0.0584769539, 0)
( 0.0596593186, 0)
( 0.0608416834, 0)
( 0.0620240481, 0)
( 0.0632064128, 0)
( 0.0643887776, 0)
( 0.0655711423, 0)
( 0.066753507, 0)
( 0.0679358717, 0)
( 0.0691182365, 0)
( 0.0703006012, 0)
( 0.0714829659, 0)
( 0.0726653307, 0)
( 0.0738476954, 0)
( 0.0750300601, 0)
( 0.0762124248, 0)
( 0.0773947896, 0)
( 0.0785771543, 0)
( 0.079759519, 0)
( 0.0809418838, 0)
( 0.0821242485, 0)
( 0.0833066132, 0)
( 0.084488978, 0)
( 0.0856713427, 0)
( 0.0868537074, 0)
( 0.0880360721, 0)
( 0.0892184369, 0)
( 0.0904008016, 0)
( 0.0915831663, 0)
( 0.0927655311, 0)
( 0.0939478958, 0)
( 0.0951302605, 0)
( 0.0963126253, 0)
( 0.09749499, 0)
( 0.0986773547, 0)
( 0.0998597194, 0)
( 0.101042084, 0)
( 0.102224449, 0)
( 0.103406814, 0)
( 0.104589178, 0)
( 0.105771543, 0)
( 0.106953908, 0)
( 0.108136273, 0)
( 0.109318637, 0)
( 0.110501002, 0)
( 0.111683367, 0)
( 0.112865731, 0)
( 0.114048096, 0)
( 0.115230461, 0)
( 0.116412826, 0)
( 0.11759519, 0)
( 0.118777555, 0)
( 0.11995992, 0)
( 0.121142285, 0)
( 0.122324649, 0)
( 0.123507014, 0)
( 0.124689379, 0)
( 0.125871743, 0)
( 0.127054108, 0)
( 0.128236473, 0)
( 0.129418838, 0)
( 0.130601202, 0)
( 0.131783567, 0)
( 0.132965932, 0)
( 0.134148297, 0)
( 0.135330661, 2.82384927e-302)
( 0.136513026, 1.80812894e-279)
( 0.137695391, 5.77937689e-258)
( 0.138877756, 9.77950449e-238)
( 0.14006012, 9.41343507e-219)
( 0.141242485, 5.60115215e-201)
( 0.14242485, 2.26001397e-184)
( 0.143607214, 6.83594357e-169)
( 0.144789579, 1.7238771e-154)
( 0.145971944, 4.04892903e-141)
( 0.147154309, 9.92469329e-129)
( 0.148336673, 2.84967115e-117)
( 0.149519038, 1.07636412e-106)
( 0.150701403, 6.00305381e-97)
( 0.151883768, 5.54085873e-88)
( 0.153066132, 9.46588503e-80)
( 0.154248497, 3.33789857e-72)
( 0.155430862, 2.70016065e-65)
( 0.156613226, 5.54791605e-59)
( 0.157795591, 3.19236372e-53)
( 0.158977956, 5.64741411e-48)
( 0.160160321, 3.35642911e-43)
( 0.161342685, 7.28977073e-39)
( 0.16252505, 6.26388509e-35)
( 0.163707415, 2.29470148e-31)
( 0.16488978, 3.84432196e-28)
( 0.166072144, 3.14502357e-25)
( 0.167254509, 1.33577298e-22)
( 0.168436874, 3.11815936e-20)
( 0.169619238, 4.21796469e-18)
( 0.170801603, 3.47244655e-16)
( 0.171983968, 1.82042701e-14)
( 0.173166333, 6.33672307e-13)
( 0.174348697, 1.52200109e-11)
( 0.175531062, 2.61318473e-10)
( 0.176713427, 3.31284709e-9)
( 0.177895792, 3.19438677e-8)
( 0.179078156, 2.40710402e-7)
( 0.180260521, 1.4529653e-6)
( 0.181442886, 7.18522542e-6)
( 0.182625251, 2.97121074e-5)
( 0.183807615, 0.000104663894)
( 0.18498998, 0.000319401485)
( 0.186172345, 0.000857362362)
( 0.187354709, 0.00205235269)
( 0.188537074, 0.00443596193)
( 0.189719439, 0.00875438483)
( 0.190901804, 0.0159342498)
( 0.192084168, 0.026991546)
( 0.193266533, 0.042897516)
( 0.194448898, 0.0644311999)
( 0.195631263, 0.0920532537)
( 0.196813627, 0.125828617)
( 0.197995992, 0.165410836)
( 0.199178357, 0.210084818)
( 0.200360721, 0.258852802)
( 0.201543086, 0.310542816)
( 0.202725451, 0.363919505)
( 0.203907816, 0.417781818)
( 0.20509018, 0.471038351)
( 0.206272545, 0.522757068)
( 0.20745491, 0.57219069)
( 0.208637275, 0.618781789)
( 0.209819639, 0.662152848)
( 0.211002004, 0.702086543)
( 0.212184369, 0.738500826)
( 0.213366733, 0.771422369)
( 0.214549098, 0.800960894)
( 0.215731463, 0.827285931)
( 0.216913828, 0.850606853)
( 0.218096192, 0.871156428)
( 0.219278557, 0.889177811)
( 0.220460922, 0.90491465)
( 0.221643287, 0.918603873)
( 0.222825651, 0.930470722)
( 0.224008016, 0.940725568)
( 0.225190381, 0.949562121)
( 0.226372745, 0.957156691)
( 0.22755511, 0.963668204)
( 0.228737475, 0.969238764)
( 0.22991984, 0.97399455)
( 0.231102204, 0.978046941)
( 0.232284569, 0.981493747)
( 0.233466934, 0.984420475)
( 0.234649299, 0.986901582)
( 0.235831663, 0.989001672)
( 0.237014028, 0.990776627)
( 0.238196393, 0.992274644)
( 0.239378758, 0.993537187)
( 0.240561122, 0.994599844)
( 0.241743487, 0.995493089)
( 0.242925852, 0.996242971)
( 0.244108216, 0.996871707)
( 0.245290581, 0.997398216)
( 0.246472946, 0.997838581)
( 0.247655311, 0.998206454)
( 0.248837675, 0.998513399)
( 0.25002004, 0.998769205)
( 0.251202405, 0.998982141)
( 0.25238477, 0.999159183)
( 0.253567134, 0.999306212)
( 0.254749499, 0.999428172)
( 0.255931864, 0.999529222)
( 0.257114228, 0.999612849)
( 0.258296593, 0.999681978)
( 0.259478958, 0.999739057)
( 0.260661323, 0.999786131)
( 0.261843687, 0.99982491)
( 0.263026052, 0.999856818)
( 0.264208417, 0.999883044)
( 0.265390782, 0.999904573)
( 0.266573146, 0.999922227)
( 0.267755511, 0.999936687)
( 0.268937876, 0.999948517)
( 0.27012024, 0.999958183)
( 0.271302605, 0.999966073)
( 0.27248497, 0.999972506)
( 0.273667335, 0.999977744)
( 0.274849699, 0.999982005)
( 0.276032064, 0.999985467)
( 0.277214429, 0.999988276)
( 0.278396794, 0.999990553)
( 0.279579158, 0.999992397)
( 0.280761523, 0.999993887)
( 0.281943888, 0.999995091)
( 0.283126253, 0.999996063)
( 0.284308617, 0.999996846)
( 0.285490982, 0.999997476)
( 0.286673347, 0.999997982)
( 0.287855711, 0.999998389)
( 0.289038076, 0.999998716)
( 0.290220441, 0.999998977)
( 0.291402806, 0.999999186)
( 0.29258517, 0.999999353)
( 0.293767535, 0.999999487)
( 0.2949499, 0.999999593)
( 0.296132265, 0.999999678)
( 0.297314629, 0.999999745)
( 0.298496994, 0.999999799)
( 0.299679359, 0.999999841)
( 0.300861723, 0.999999875)
( 0.302044088, 0.999999901)
( 0.303226453, 0.999999922)
( 0.304408818, 0.999999939)
( 0.305591182, 0.999999952)
( 0.306773547, 0.999999962)
( 0.307955912, 0.999999971)
( 0.309138277, 0.999999977)
( 0.310320641, 0.999999982)
( 0.311503006, 0.999999986)
( 0.312685371, 0.999999989)
( 0.313867735, 0.999999992)
( 0.3150501, 0.999999993)
( 0.316232465, 0.999999995)
( 0.31741483, 0.999999996)
( 0.318597194, 0.999999997)
( 0.319779559, 0.999999998)
( 0.320961924, 0.999999998)
( 0.322144289, 0.999999999)
( 0.323326653, 0.999999999)
( 0.324509018, 0.999999999)
( 0.325691383, 0.999999999)
( 0.326873747, 0.999999999)
( 0.328056112, 1)
( 0.329238477, 1)
( 0.330420842, 1)
( 0.331603206, 1)
( 0.332785571, 1)
( 0.333967936, 1)
( 0.335150301, 1)
( 0.336332665, 1)
( 0.33751503, 1)
( 0.338697395, 1)
( 0.33987976, 1)
( 0.341062124, 1)
( 0.342244489, 1)
( 0.343426854, 1)
( 0.344609218, 1)
( 0.345791583, 1)
( 0.346973948, 1)
( 0.348156313, 1)
( 0.349338677, 1)
( 0.350521042, 1)
( 0.351703407, 1)
( 0.352885772, 1)
( 0.354068136, 1)
( 0.355250501, 1)
( 0.356432866, 1)
( 0.35761523, 1)
( 0.358797595, 1)
( 0.35997996, 1)
( 0.361162325, 1)
( 0.362344689, 1)
( 0.363527054, 1)
( 0.364709419, 1)
( 0.365891784, 1)
( 0.367074148, 1)
( 0.368256513, 1)
( 0.369438878, 1)
( 0.370621242, 1)
( 0.371803607, 1)
( 0.372985972, 1)
( 0.374168337, 1)
( 0.375350701, 1)
( 0.376533066, 1)
( 0.377715431, 1)
( 0.378897796, 1)
( 0.38008016, 1)
( 0.381262525, 1)
( 0.38244489, 1)
( 0.383627255, 1)
( 0.384809619, 1)
( 0.385991984, 1)
( 0.387174349, 1)
( 0.388356713, 1)
( 0.389539078, 1)
( 0.390721443, 1)
( 0.391903808, 1)
( 0.393086172, 1)
( 0.394268537, 1)
( 0.395450902, 1)
( 0.396633267, 1)
( 0.397815631, 1)
( 0.398997996, 1)
( 0.400180361, 1)
( 0.401362725, 1)
( 0.40254509, 1)
( 0.403727455, 1)
( 0.40490982, 1)
( 0.406092184, 1)
( 0.407274549, 1)
( 0.408456914, 1)
( 0.409639279, 1)
( 0.410821643, 1)
( 0.412004008, 1)
( 0.413186373, 1)
( 0.414368737, 1)
( 0.415551102, 1)
( 0.416733467, 1)
( 0.417915832, 1)
( 0.419098196, 1)
( 0.420280561, 1)
( 0.421462926, 1)
( 0.422645291, 1)
( 0.423827655, 1)
( 0.42501002, 1)
( 0.426192385, 1)
( 0.427374749, 1)
( 0.428557114, 1)
( 0.429739479, 1)
( 0.430921844, 1)
( 0.432104208, 1)
( 0.433286573, 1)
( 0.434468938, 1)
( 0.435651303, 1)
( 0.436833667, 1)
( 0.438016032, 1)
( 0.439198397, 1)
( 0.440380762, 1)
( 0.441563126, 1)
( 0.442745491, 1)
( 0.443927856, 1)
( 0.44511022, 1)
( 0.446292585, 1)
( 0.44747495, 1)
( 0.448657315, 1)
( 0.449839679, 1)
( 0.451022044, 1)
( 0.452204409, 1)
( 0.453386774, 1)
( 0.454569138, 1)
( 0.455751503, 1)
( 0.456933868, 1)
( 0.458116232, 1)
( 0.459298597, 1)
( 0.460480962, 1)
( 0.461663327, 1)
( 0.462845691, 1)
( 0.464028056, 1)
( 0.465210421, 1)
( 0.466392786, 1)
( 0.46757515, 1)
( 0.468757515, 1)
( 0.46993988, 1)
( 0.471122244, 1)
( 0.472304609, 1)
( 0.473486974, 1)
( 0.474669339, 1)
( 0.475851703, 1)
( 0.477034068, 1)
( 0.478216433, 1)
( 0.479398798, 1)
( 0.480581162, 1)
( 0.481763527, 1)
( 0.482945892, 1)
( 0.484128257, 1)
( 0.485310621, 1)
( 0.486492986, 1)
( 0.487675351, 1)
( 0.488857715, 1)
( 0.49004008, 1)
( 0.491222445, 1)
( 0.49240481, 1)
( 0.493587174, 1)
( 0.494769539, 1)
( 0.495951904, 1)
( 0.497134269, 1)
( 0.498316633, 1)
( 0.499498998, 1)
( 0.500681363, 1)
( 0.501863727, 1)
( 0.503046092, 1)
( 0.504228457, 1)
( 0.505410822, 1)
( 0.506593186, 1)
( 0.507775551, 1)
( 0.508957916, 1)
( 0.510140281, 1)
( 0.511322645, 1)
( 0.51250501, 1)
( 0.513687375, 1)
( 0.514869739, 1)
( 0.516052104, 1)
( 0.517234469, 1)
( 0.518416834, 1)
( 0.519599198, 1)
( 0.520781563, 1)
( 0.521963928, 1)
( 0.523146293, 1)
( 0.524328657, 1)
( 0.525511022, 1)
( 0.526693387, 1)
( 0.527875752, 1)
( 0.529058116, 1)
( 0.530240481, 1)
( 0.531422846, 1)
( 0.53260521, 1)
( 0.533787575, 1)
( 0.53496994, 1)
( 0.536152305, 1)
( 0.537334669, 1)
( 0.538517034, 1)
( 0.539699399, 1)
( 0.540881764, 1)
( 0.542064128, 1)
( 0.543246493, 1)
( 0.544428858, 1)
( 0.545611222, 1)
( 0.546793587, 1)
( 0.547975952, 1)
( 0.549158317, 1)
( 0.550340681, 1)
( 0.551523046, 1)
( 0.552705411, 1)
( 0.553887776, 1)
( 0.55507014, 1)
( 0.556252505, 1)
( 0.55743487, 1)
( 0.558617234, 1)
( 0.559799599, 1)
( 0.560981964, 1)
( 0.562164329, 1)
( 0.563346693, 1)
( 0.564529058, 1)
( 0.565711423, 1)
( 0.566893788, 1)
( 0.568076152, 1)
( 0.569258517, 1)
( 0.570440882, 1)
( 0.571623246, 1)
( 0.572805611, 1)
( 0.573987976, 1)
( 0.575170341, 1)
( 0.576352705, 1)
( 0.57753507, 1)
( 0.578717435, 1)
( 0.5798998, 1)
( 0.581082164, 1)
( 0.582264529, 1)
( 0.583446894, 1)
( 0.584629259, 1)
( 0.585811623, 1)
( 0.586993988, 1)
( 0.588176353, 1)
( 0.589358717, 1)
( 0.590541082, 1)
( 0.591723447, 1)
( 0.592905812, 1)
( 0.594088176, 1)
( 0.595270541, 1)
( 0.596452906, 1)
( 0.597635271, 1)
( 0.598817635, 1)
( 0.6, 1)
};
\addplot [blue ,dashed]
coordinates {
( 0.01, 0)
( 0.013877551, 0)
( 0.017755102, 0)
( 0.021632653, 0)
( 0.025510204, 0)
( 0.029387755, 0)
( 0.033265306, 0)
( 0.037142857, 0)
( 0.041020408, 0)
( 0.044897959, 0)
( 0.04877551, 0)
( 0.052653061, 0)
( 0.056530612, 0)
( 0.060408163, 0)
( 0.064285714, 0)
( 0.068163265, 0)
( 0.072040816, 0)
( 0.075918367, 0)
( 0.079795918, 0)
( 0.083673469, 0)
( 0.08755102, 0)
( 0.091428571, 0)
( 0.095306122, 0)
( 0.099183673, 0)
( 0.10306122, 0)
( 0.10693878, 0)
( 0.11081633, 0)
( 0.11469388, 0)
( 0.11857143, 0.01)
( 0.12244898, 0.1575)
( 0.12632653, 0.4825)
( 0.13020408, 0.74)
( 0.13408163, 0.9)
( 0.13795918, 0.9575)
( 0.14183673, 0.9825)
( 0.14571429, 1)
( 0.14959184, 0.9975)
( 0.15346939, 0.9975)
( 0.15734694, 1)
( 0.16122449, 1)
( 0.16510204, 1)
( 0.16897959, 1)
( 0.17285714, 1)
( 0.17673469, 1)
( 0.18061224, 1)
( 0.1844898, 1)
( 0.18836735, 1)
( 0.1922449, 1)
( 0.19612245, 1)
( 0.2, 1)
( 0.3, 1)
( 0.6, 1)
( 0.99, 1)
};
\draw (axis cs:  0.42, 0.2) node {32  };
\draw (axis cs:  0.345, 0.4) node {100 };
\draw (axis cs:  0.235, 0.6) node {316 };
\draw (axis cs:  0.16, 0.8) node {1000};
\addplot [dash dot]
coordinates {
( 0.01, 0)
( 0.0111823647, 0)
( 0.0123647295, 0)
( 0.0135470942, 0)
( 0.0147294589, 0)
( 0.0159118236, 0)
( 0.0170941884, 0)
( 0.0182765531, 0)
( 0.0194589178, 0)
( 0.0206412826, 0)
( 0.0218236473, 0)
( 0.023006012, 0)
( 0.0241883768, 0)
( 0.0253707415, 0)
( 0.0265531062, 0)
( 0.0277354709, 0)
( 0.0289178357, 0)
( 0.0301002004, 0)
( 0.0312825651, 0)
( 0.0324649299, 0)
( 0.0336472946, 0)
( 0.0348296593, 0)
( 0.036012024, 0)
( 0.0371943888, 0)
( 0.0383767535, 0)
( 0.0395591182, 0)
( 0.040741483, 0)
( 0.0419238477, 0)
( 0.0431062124, 0)
( 0.0442885772, 0)
( 0.0454709419, 0)
( 0.0466533066, 0)
( 0.0478356713, 0)
( 0.0490180361, 0)
( 0.0502004008, 0)
( 0.0513827655, 0)
( 0.0525651303, 0)
( 0.053747495, 0)
( 0.0549298597, 0)
( 0.0561122244, 0)
( 0.0572945892, 0)
( 0.0584769539, 0)
( 0.0596593186, 0)
( 0.0608416834, 0)
( 0.0620240481, 0)
( 0.0632064128, 0)
( 0.0643887776, 0)
( 0.0655711423, 0)
( 0.066753507, 0)
( 0.0679358717, 0)
( 0.0691182365, 0)
( 0.0703006012, 0)
( 0.0714829659, 0)
( 0.0726653307, 0)
( 0.0738476954, 0)
( 0.0750300601, 0)
( 0.0762124248, 0)
( 0.0773947896, 0)
( 0.0785771543, 0)
( 0.079759519, 0)
( 0.0809418838, 3.37735333e-283)
( 0.0821242485, 3.96222462e-233)
( 0.0833066132, 2.15088544e-191)
( 0.084488978, 1.03603372e-156)
( 0.0856713427, 5.63666197e-128)
( 0.0868537074, 3.07352227e-104)
( 0.0880360721, 1.08600467e-84)
( 0.0892184369, 1.2195061e-68)
( 0.0904008016, 1.67836605e-55)
( 0.0915831663, 8.86633758e-45)
( 0.0927655311, 4.70558278e-36)
( 0.0939478958, 5.62868736e-29)
( 0.0951302605, 2.98385799e-23)
( 0.0963126253, 1.2319648e-18)
( 0.09749499, 6.32917577e-15)
( 0.0986773547, 5.9637557e-12)
( 0.0998597194, 1.41957429e-9)
( 0.101042084, 1.11071548e-7)
( 0.102224449, 3.54453093e-6)
( 0.103406814, 5.50245254e-5)
( 0.104589178, 0.000479607514)
( 0.105771543, 0.00263679247)
( 0.106953908, 0.0100455665)
( 0.108136273, 0.0286083505)
( 0.109318637, 0.0647230135)
( 0.110501002, 0.122129989)
( 0.111683367, 0.199826762)
( 0.112865731, 0.292391062)
( 0.114048096, 0.392084814)
( 0.115230461, 0.491239533)
( 0.116412826, 0.58386079)
( 0.11759519, 0.666208361)
( 0.118777555, 0.736627114)
( 0.11995992, 0.795024124)
( 0.121142285, 0.842289228)
( 0.122324649, 0.879812541)
( 0.123507014, 0.909144894)
( 0.124689379, 0.931789762)
( 0.125871743, 0.949094419)
( 0.127054108, 0.962206979)
( 0.128236473, 0.972072592)
( 0.129418838, 0.979450186)
( 0.130601202, 0.984937939)
( 0.131783567, 0.989000658)
( 0.132965932, 0.991995486)
( 0.134148297, 0.994194374)
( 0.135330661, 0.995802859)
( 0.136513026, 0.996975306)
( 0.137695391, 0.997827016)
( 0.138877756, 0.998443688)
( 0.14006012, 0.998888743)
( 0.141242485, 0.999208923)
( 0.14242485, 0.999438544)
( 0.143607214, 0.999602709)
( 0.144789579, 0.999719714)
( 0.145971944, 0.99980285)
( 0.147154309, 0.999861742)
( 0.148336673, 0.999903331)
( 0.149519038, 0.999932611)
( 0.150701403, 0.999953163)
( 0.151883768, 0.999967544)
( 0.153066132, 0.999977577)
( 0.154248497, 0.999984555)
( 0.155430862, 0.999989393)
( 0.156613226, 0.999992738)
( 0.157795591, 0.999995043)
( 0.158977956, 0.999996626)
( 0.160160321, 0.999997711)
( 0.161342685, 0.999998451)
( 0.16252505, 0.999998955)
( 0.163707415, 0.999999298)
( 0.16488978, 0.999999529)
( 0.166072144, 0.999999685)
( 0.167254509, 0.99999979)
( 0.168436874, 0.999999861)
( 0.169619238, 0.999999908)
( 0.170801603, 0.999999939)
( 0.171983968, 0.99999996)
( 0.173166333, 0.999999974)
( 0.174348697, 0.999999983)
( 0.175531062, 0.999999989)
( 0.176713427, 0.999999993)
( 0.177895792, 0.999999995)
( 0.179078156, 0.999999997)
( 0.180260521, 0.999999998)
( 0.181442886, 0.999999999)
( 0.182625251, 0.999999999)
( 0.183807615, 1)
( 0.18498998, 1)
( 0.186172345, 1)
( 0.187354709, 1)
( 0.188537074, 1)
( 0.189719439, 1)
( 0.190901804, 1)
( 0.192084168, 1)
( 0.193266533, 1)
( 0.194448898, 1)
( 0.195631263, 1)
( 0.196813627, 1)
( 0.197995992, 1)
( 0.199178357, 1)
( 0.200360721, 1)
( 0.201543086, 1)
( 0.202725451, 1)
( 0.203907816, 1)
( 0.20509018, 1)
( 0.206272545, 1)
( 0.20745491, 1)
( 0.208637275, 1)
( 0.209819639, 1)
( 0.211002004, 1)
( 0.212184369, 1)
( 0.213366733, 1)
( 0.214549098, 1)
( 0.215731463, 1)
( 0.216913828, 1)
( 0.218096192, 1)
( 0.219278557, 1)
( 0.220460922, 1)
( 0.221643287, 1)
( 0.222825651, 1)
( 0.224008016, 1)
( 0.225190381, 1)
( 0.226372745, 1)
( 0.22755511, 1)
( 0.228737475, 1)
( 0.22991984, 1)
( 0.231102204, 1)
( 0.232284569, 1)
( 0.233466934, 1)
( 0.234649299, 1)
( 0.235831663, 1)
( 0.237014028, 1)
( 0.238196393, 1)
( 0.239378758, 1)
( 0.240561122, 1)
( 0.241743487, 1)
( 0.242925852, 1)
( 0.244108216, 1)
( 0.245290581, 1)
( 0.246472946, 1)
( 0.247655311, 1)
( 0.248837675, 1)
( 0.25002004, 1)
( 0.251202405, 1)
( 0.25238477, 1)
( 0.253567134, 1)
( 0.254749499, 1)
( 0.255931864, 1)
( 0.257114228, 1)
( 0.258296593, 1)
( 0.259478958, 1)
( 0.260661323, 1)
( 0.261843687, 1)
( 0.263026052, 1)
( 0.264208417, 1)
( 0.265390782, 1)
( 0.266573146, 1)
( 0.267755511, 1)
( 0.268937876, 1)
( 0.27012024, 1)
( 0.271302605, 1)
( 0.27248497, 1)
( 0.273667335, 1)
( 0.274849699, 1)
( 0.276032064, 1)
( 0.277214429, 1)
( 0.278396794, 1)
( 0.279579158, 1)
( 0.280761523, 1)
( 0.281943888, 1)
( 0.283126253, 1)
( 0.284308617, 1)
( 0.285490982, 1)
( 0.286673347, 1)
( 0.287855711, 1)
( 0.289038076, 1)
( 0.290220441, 1)
( 0.291402806, 1)
( 0.29258517, 1)
( 0.293767535, 1)
( 0.2949499, 1)
( 0.296132265, 1)
( 0.297314629, 1)
( 0.298496994, 1)
( 0.299679359, 1)
( 0.300861723, 1)
( 0.302044088, 1)
( 0.303226453, 1)
( 0.304408818, 1)
( 0.305591182, 1)
( 0.306773547, 1)
( 0.307955912, 1)
( 0.309138277, 1)
( 0.310320641, 1)
( 0.311503006, 1)
( 0.312685371, 1)
( 0.313867735, 1)
( 0.3150501, 1)
( 0.316232465, 1)
( 0.31741483, 1)
( 0.318597194, 1)
( 0.319779559, 1)
( 0.320961924, 1)
( 0.322144289, 1)
( 0.323326653, 1)
( 0.324509018, 1)
( 0.325691383, 1)
( 0.326873747, 1)
( 0.328056112, 1)
( 0.329238477, 1)
( 0.330420842, 1)
( 0.331603206, 1)
( 0.332785571, 1)
( 0.333967936, 1)
( 0.335150301, 1)
( 0.336332665, 1)
( 0.33751503, 1)
( 0.338697395, 1)
( 0.33987976, 1)
( 0.341062124, 1)
( 0.342244489, 1)
( 0.343426854, 1)
( 0.344609218, 1)
( 0.345791583, 1)
( 0.346973948, 1)
( 0.348156313, 1)
( 0.349338677, 1)
( 0.350521042, 1)
( 0.351703407, 1)
( 0.352885772, 1)
( 0.354068136, 1)
( 0.355250501, 1)
( 0.356432866, 1)
( 0.35761523, 1)
( 0.358797595, 1)
( 0.35997996, 1)
( 0.361162325, 1)
( 0.362344689, 1)
( 0.363527054, 1)
( 0.364709419, 1)
( 0.365891784, 1)
( 0.367074148, 1)
( 0.368256513, 1)
( 0.369438878, 1)
( 0.370621242, 1)
( 0.371803607, 1)
( 0.372985972, 1)
( 0.374168337, 1)
( 0.375350701, 1)
( 0.376533066, 1)
( 0.377715431, 1)
( 0.378897796, 1)
( 0.38008016, 1)
( 0.381262525, 1)
( 0.38244489, 1)
( 0.383627255, 1)
( 0.384809619, 1)
( 0.385991984, 1)
( 0.387174349, 1)
( 0.388356713, 1)
( 0.389539078, 1)
( 0.390721443, 1)
( 0.391903808, 1)
( 0.393086172, 1)
( 0.394268537, 1)
( 0.395450902, 1)
( 0.396633267, 1)
( 0.397815631, 1)
( 0.398997996, 1)
( 0.400180361, 1)
( 0.401362725, 1)
( 0.40254509, 1)
( 0.403727455, 1)
( 0.40490982, 1)
( 0.406092184, 1)
( 0.407274549, 1)
( 0.408456914, 1)
( 0.409639279, 1)
( 0.410821643, 1)
( 0.412004008, 1)
( 0.413186373, 1)
( 0.414368737, 1)
( 0.415551102, 1)
( 0.416733467, 1)
( 0.417915832, 1)
( 0.419098196, 1)
( 0.420280561, 1)
( 0.421462926, 1)
( 0.422645291, 1)
( 0.423827655, 1)
( 0.42501002, 1)
( 0.426192385, 1)
( 0.427374749, 1)
( 0.428557114, 1)
( 0.429739479, 1)
( 0.430921844, 1)
( 0.432104208, 1)
( 0.433286573, 1)
( 0.434468938, 1)
( 0.435651303, 1)
( 0.436833667, 1)
( 0.438016032, 1)
( 0.439198397, 1)
( 0.440380762, 1)
( 0.441563126, 1)
( 0.442745491, 1)
( 0.443927856, 1)
( 0.44511022, 1)
( 0.446292585, 1)
( 0.44747495, 1)
( 0.448657315, 1)
( 0.449839679, 1)
( 0.451022044, 1)
( 0.452204409, 1)
( 0.453386774, 1)
( 0.454569138, 1)
( 0.455751503, 1)
( 0.456933868, 1)
( 0.458116232, 1)
( 0.459298597, 1)
( 0.460480962, 1)
( 0.461663327, 1)
( 0.462845691, 1)
( 0.464028056, 1)
( 0.465210421, 1)
( 0.466392786, 1)
( 0.46757515, 1)
( 0.468757515, 1)
( 0.46993988, 1)
( 0.471122244, 1)
( 0.472304609, 1)
( 0.473486974, 1)
( 0.474669339, 1)
( 0.475851703, 1)
( 0.477034068, 1)
( 0.478216433, 1)
( 0.479398798, 1)
( 0.480581162, 1)
( 0.481763527, 1)
( 0.482945892, 1)
( 0.484128257, 1)
( 0.485310621, 1)
( 0.486492986, 1)
( 0.487675351, 1)
( 0.488857715, 1)
( 0.49004008, 1)
( 0.491222445, 1)
( 0.49240481, 1)
( 0.493587174, 1)
( 0.494769539, 1)
( 0.495951904, 1)
( 0.497134269, 1)
( 0.498316633, 1)
( 0.499498998, 1)
( 0.500681363, 1)
( 0.501863727, 1)
( 0.503046092, 1)
( 0.504228457, 1)
( 0.505410822, 1)
( 0.506593186, 1)
( 0.507775551, 1)
( 0.508957916, 1)
( 0.510140281, 1)
( 0.511322645, 1)
( 0.51250501, 1)
( 0.513687375, 1)
( 0.514869739, 1)
( 0.516052104, 1)
( 0.517234469, 1)
( 0.518416834, 1)
( 0.519599198, 1)
( 0.520781563, 1)
( 0.521963928, 1)
( 0.523146293, 1)
( 0.524328657, 1)
( 0.525511022, 1)
( 0.526693387, 1)
( 0.527875752, 1)
( 0.529058116, 1)
( 0.530240481, 1)
( 0.531422846, 1)
( 0.53260521, 1)
( 0.533787575, 1)
( 0.53496994, 1)
( 0.536152305, 1)
( 0.537334669, 1)
( 0.538517034, 1)
( 0.539699399, 1)
( 0.540881764, 1)
( 0.542064128, 1)
( 0.543246493, 1)
( 0.544428858, 1)
( 0.545611222, 1)
( 0.546793587, 1)
( 0.547975952, 1)
( 0.549158317, 1)
( 0.550340681, 1)
( 0.551523046, 1)
( 0.552705411, 1)
( 0.553887776, 1)
( 0.55507014, 1)
( 0.556252505, 1)
( 0.55743487, 1)
( 0.558617234, 1)
( 0.559799599, 1)
( 0.560981964, 1)
( 0.562164329, 1)
( 0.563346693, 1)
( 0.564529058, 1)
( 0.565711423, 1)
( 0.566893788, 1)
( 0.568076152, 1)
( 0.569258517, 1)
( 0.570440882, 1)
( 0.571623246, 1)
( 0.572805611, 1)
( 0.573987976, 1)
( 0.575170341, 1)
( 0.576352705, 1)
( 0.57753507, 1)
( 0.578717435, 1)
( 0.5798998, 1)
( 0.581082164, 1)
( 0.582264529, 1)
( 0.583446894, 1)
( 0.584629259, 1)
( 0.585811623, 1)
( 0.586993988, 1)
( 0.588176353, 1)
( 0.589358717, 1)
( 0.590541082, 1)
( 0.591723447, 1)
( 0.592905812, 1)
( 0.594088176, 1)
( 0.595270541, 1)
( 0.596452906, 1)
( 0.597635271, 1)
( 0.598817635, 1)
( 0.6, 1)
};
\end{axis}


==> Gnpthreshold.tex <==
\begin{loglogaxis}[
xlabel={$n$},
ylabel={$p$},
ylabel near ticks,
]
\addplot [dotted]
coordinates {
( 1000, 0.00690775528)
( 1623.77674, 0.00455266408)
( 2636.6509, 0.00298760249)
( 4281.3324, 0.00195313486)
( 6951.92796, 0.00127256415)
( 11288.3789, 0.00082664917)
( 18329.8071, 0.000535536668)
( 29763.5144, 0.000346096178)
( 48329.3024, 0.000223172957)
( 78475.997, 0.000143617775)
( 127427.499, 9.22509111e-5)
( 206913.808, 5.91553445e-5)
( 335981.829, 3.78735136e-5)
( 545559.478, 2.42128817e-5)
( 885866.79, 1.54586694e-5)
( 1438449.89, 9.85719193e-6)
( 2335721.47, 6.27807364e-6)
( 3792690.19, 3.99415333e-6)
( 6158482.11, 2.53850553e-6)
( 10000000, 1.61180957e-6)
};
\addplot [ ]
coordinates {
( 1000, 0.0086346941)
( 1623.77674, 0.0056908301)
( 2636.6509, 0.00373450311)
( 4281.3324, 0.00244141857)
( 6951.92796, 0.00159070519)
( 11288.3789, 0.00103331146)
( 18329.8071, 0.000669420835)
( 29763.5144, 0.000432620222)
( 48329.3024, 0.000278966196)
( 78475.997, 0.000179522219)
( 127427.499, 0.000115313639)
( 206913.808, 7.39441806e-5)
( 335981.829, 4.7341892e-5)
( 545559.478, 3.02661021e-5)
( 885866.79, 1.93233368e-5)
( 1438449.89, 1.23214899e-5)
( 2335721.47, 7.84759205e-6)
( 3792690.19, 4.99269166e-6)
( 6158482.11, 3.17313191e-6)
( 10000000, 2.01476196e-6)
};
\addplot [ ]
coordinates {
( 1000, 0.0831129068)
( 1623.77674, 0.0674734324)
( 2636.6509, 0.0546589653)
( 4281.3324, 0.0441942854)
( 6951.92796, 0.0356730171)
( 11288.3789, 0.0287515073)
( 18329.8071, 0.0231416652)
( 29763.5144, 0.0186036603)
( 48329.3024, 0.0149389744)
( 78475.997, 0.0119840634)
( 127427.499, 0.00960473379)
( 206913.808, 0.00769125117)
( 335981.829, 0.00615414605)
( 545559.478, 0.00492065867)
( 885866.79, 0.00393175145)
( 1438449.89, 0.00313961653)
( 2335721.47, 0.00250560844)
( 3792690.19, 0.0019985378)
( 6158482.11, 0.00159326882)
( 10000000, 0.00126957062)
};
\addplot [ dashed]
coordinates {
( 1000, 0.1175394)
( 1623.77674, 0.0954218432)
( 2636.6509, 0.0772994501)
( 4281.3324, 0.0625001577)
( 6951.92796, 0.0504492646)
( 11288.3789, 0.0406607715)
( 18329.8071, 0.0327272568)
( 29763.5144, 0.0263095487)
( 48329.3024, 0.0211269003)
( 78475.997, 0.016948025)
( 127427.499, 0.0135831448)
( 206913.808, 0.0108770717)
( 335981.829, 0.00870327681)
( 545559.478, 0.00695886222)
( 885866.79, 0.00556033622)
( 1438449.89, 0.00444008827)
( 2335721.47, 0.00354346543)
( 3792690.19, 0.00282635926)
( 6158482.11, 0.00225322237)
( 10000000, 0.00179544399)
};
\addplot [ dash dot]
coordinates {
( 1000, 0.131413044)
( 1623.77674, 0.106684864)
( 2636.6509, 0.0864234125)
( 4281.3324, 0.0698773006)
( 6951.92796, 0.0564039926)
( 11288.3789, 0.0454601246)
( 18329.8071, 0.0365901854)
( 29763.5144, 0.0294149697)
( 48329.3024, 0.0236205926)
( 78475.997, 0.0189484679)
( 127427.499, 0.0151864175)
( 206913.808, 0.0121609359)
( 335981.829, 0.00973055929)
( 545559.478, 0.00778024449)
( 885866.79, 0.00621664488)
( 1438449.89, 0.0049641696)
( 2335721.47, 0.00396171479)
( 3792690.19, 0.00315996571)
( 6158482.11, 0.0025191792)
( 10000000, 0.00200736741)
};
\draw (axis cs:  10000, 0.0001) node {disconnected};
\draw (axis cs:  40000, 0.003) node {weak        };
\draw (axis cs:  300000, 0.1) node {strong      };
\end{loglogaxis}


==> Gnpweak.tex <==
\begin{axis}[
xmin= 0, xmax= 0.5,
xlabel={$p$},
ylabel={$P$(weak)},
ylabel near ticks,
]
\addplot [black,]
coordinates {
( 0.05, 0)
( 0.06122449, 0)
( 0.07244898, 0.00087336245)
( 0.083673469, 0)
( 0.094897959, 0)
( 0.10612245, 0.000625)
( 0.11734694, 0.00125)
( 0.12857143, 0.006875)
( 0.13979592, 0.00625)
( 0.15102041, 0.00875)
( 0.1622449, 0.013125)
( 0.17346939, 0.0125)
( 0.18469388, 0.01375)
( 0.19591837, 0.0125)
( 0.20714286, 0.011875)
( 0.21836735, 0.010625)
( 0.22959184, 0.010625)
( 0.24081633, 0.005)
( 0.25204082, 0.001875)
( 0.26326531, 0.00125)
( 0.2744898, 0.00125)
( 0.28571429, 0.000625)
( 0.29693878, 0.000625)
( 0.30816327, 0)
( 0.31938776, 0)
( 0.33061224, 0)
( 0.34183673, 0)
( 0.35306122, 0)
( 0.36428571, 0)
( 0.3755102, 0)
( 0.38673469, 0)
( 0.39795918, 0)
( 0.40918367, 0)
( 0.42040816, 0)
( 0.43163265, 0)
( 0.44285714, 0)
( 0.45408163, 0)
( 0.46530612, 0)
( 0.47653061, 0)
( 0.4877551, 0)
( 0.49897959, 0)
( 0.51020408, 0)
( 0.52142857, 0)
( 0.53265306, 0)
( 0.54387755, 0)
( 0.55510204, 0)
( 0.56632653, 0)
( 0.57755102, 0)
( 0.58877551, 0)
( 0.6, 0)
( 0.7, 0)
( 0.9, 0)
( 0.99, 0)
};
\addplot [black,dotted]
coordinates {
( 0.01, 2.55263943e-47)
( 0.0111823647, 1.45627802e-44)
( 0.0123647295, 4.05495768e-42)
( 0.0135470942, 6.28672132e-40)
( 0.0147294589, 5.98941717e-38)
( 0.0159118236, 3.78237646e-36)
( 0.0170941884, 1.68029461e-34)
( 0.0182765531, 5.50664323e-33)
( 0.0194589178, 1.38366208e-31)
( 0.0206412826, 2.75177147e-30)
( 0.0218236473, 4.4476357e-29)
( 0.023006012, 5.97392442e-28)
( 0.0241883768, 6.79565231e-27)
( 0.0253707415, 6.65420241e-26)
( 0.0265531062, 5.68782325e-25)
( 0.0277354709, 4.29615371e-24)
( 0.0289178357, 2.89824138e-23)
( 0.0301002004, 1.76275721e-22)
( 0.0312825651, 9.74688978e-22)
( 0.0324649299, 4.93591175e-21)
( 0.0336472946, 2.30444072e-20)
( 0.0348296593, 9.97777423e-20)
( 0.036012024, 4.02799008e-19)
( 0.0371943888, 1.52343086e-18)
( 0.0383767535, 5.42168206e-18)
( 0.0395591182, 1.82283538e-17)
( 0.040741483, 5.81080224e-17)
( 0.0419238477, 1.76213162e-16)
( 0.0431062124, 5.0988545e-16)
( 0.0442885772, 1.41172545e-15)
( 0.0454709419, 3.74961424e-15)
( 0.0466533066, 9.57658801e-15)
( 0.0478356713, 2.35707991e-14)
( 0.0490180361, 5.60219548e-14)
( 0.0502004008, 1.28819069e-13)
( 0.0513827655, 2.87077824e-13)
( 0.0525651303, 6.21045875e-13)
( 0.053747495, 1.30620436e-12)
( 0.0549298597, 2.67471092e-12)
( 0.0561122244, 5.33943604e-12)
( 0.0572945892, 1.04040932e-11)
( 0.0584769539, 1.98110184e-11)
( 0.0596593186, 3.69041393e-11)
( 0.0608416834, 6.73212324e-11)
( 0.0620240481, 1.20379876e-10)
( 0.0632064128, 2.11189295e-10)
( 0.0643887776, 3.63809771e-10)
( 0.0655711423, 6.15897081e-10)
( 0.066753507, 1.02541636e-9)
( 0.0679358717, 1.68019277e-9)
( 0.0691182365, 2.71128989e-9)
( 0.0703006012, 4.31147491e-9)
( 0.0714829659, 6.76034557e-9)
( 0.0726653307, 1.04580581e-8)
( 0.0738476954, 1.59700096e-8)
( 0.0750300601, 2.40852857e-8)
( 0.0762124248, 3.5892187e-8)
( 0.0773947896, 5.28746746e-8)
( 0.0785771543, 7.70341292e-8)
( 0.079759519, 1.11041371e-7)
( 0.0809418838, 1.5842443e-7)
( 0.0821242485, 2.23798045e-7)
( 0.0833066132, 3.13141346e-7)
( 0.084488978, 4.34130463e-7)
( 0.0856713427, 5.96533097e-7)
( 0.0868537074, 8.12672135e-7)
( 0.0880360721, 1.09796529e-6)
( 0.0892184369, 1.47154748e-6)
( 0.0904008016, 1.95698203e-6)
( 0.0915831663, 2.58306613e-6)
( 0.0927655311, 3.38473483e-6)
( 0.0939478958, 4.40406648e-6)
( 0.0951302605, 5.69139101e-6)
( 0.0963126253, 7.30650051e-6)
( 0.09749499, 9.31995932e-6)
( 0.0986773547, 1.18145087e-5)
( 0.0998597194, 1.48865582e-5)
( 0.101042084, 1.86477538e-5)
( 0.102224449, 2.32266087e-5)
( 0.103406814, 2.87701814e-5)
( 0.104589178, 3.54457823e-5)
( 0.105771543, 4.34426857e-5)
( 0.106953908, 5.29738242e-5)
( 0.108136273, 6.42774385e-5)
( 0.109318637, 7.76186522e-5)
( 0.110501002, 9.32909437e-5)
( 0.111683367, 0.000111617481)
( 0.112865731, 0.000132952288)
( 0.114048096, 0.000157681207)
( 0.115230461, 0.000186222635)
( 0.116412826, 0.00021902798)
( 0.11759519, 0.000256581835)
( 0.118777555, 0.000299401823)
( 0.11995992, 0.000348038093)
( 0.121142285, 0.000403072442)
( 0.122324649, 0.000465117062)
( 0.123507014, 0.000534812864)
( 0.124689379, 0.000612827413)
( 0.125871743, 0.000699852432)
( 0.127054108, 0.0007966009)
( 0.128236473, 0.000903803746)
( 0.129418838, 0.00102220614)
( 0.130601202, 0.00115256341)
( 0.131783567, 0.00129563662)
( 0.132965932, 0.00145218782)
( 0.134148297, 0.00162297495)
( 0.135330661, 0.00180874659)
( 0.136513026, 0.00201023643)
( 0.137695391, 0.00222815756)
( 0.138877756, 0.0024631967)
( 0.14006012, 0.00271600829)
( 0.141242485, 0.00298720863)
( 0.14242485, 0.00327737003)
( 0.143607214, 0.00358701499)
( 0.144789579, 0.00391661063)
( 0.145971944, 0.00426656319)
( 0.147154309, 0.00463721292)
( 0.148336673, 0.00502882906)
( 0.149519038, 0.00544160539)
( 0.150701403, 0.00587565593)
( 0.151883768, 0.00633101124)
( 0.153066132, 0.00680761501)
( 0.154248497, 0.00730532127)
( 0.155430862, 0.00782389199)
( 0.156613226, 0.00836299529)
( 0.157795591, 0.0089222041)
( 0.158977956, 0.00950099546)
( 0.160160321, 0.0100987503)
( 0.161342685, 0.0107147539)
( 0.16252505, 0.0113481965)
( 0.163707415, 0.0119981753)
( 0.16488978, 0.0126636961)
( 0.166072144, 0.0133436756)
( 0.167254509, 0.0140369449)
( 0.168436874, 0.0147422529)
( 0.169619238, 0.0154582698)
( 0.170801603, 0.0161835919)
( 0.171983968, 0.0169167463)
( 0.173166333, 0.0176561957)
( 0.174348697, 0.0184003443)
( 0.175531062, 0.019147543)
( 0.176713427, 0.0198960958)
( 0.177895792, 0.0206442657)
( 0.179078156, 0.0213902814)
( 0.180260521, 0.0221323435)
( 0.181442886, 0.0228686313)
( 0.182625251, 0.0235973096)
( 0.183807615, 0.0243165354)
( 0.18498998, 0.0250244646)
( 0.186172345, 0.0257192589)
( 0.187354709, 0.0263990928)
( 0.188537074, 0.0270621595)
( 0.189719439, 0.0277066784)
( 0.190901804, 0.0283309009)
( 0.192084168, 0.028933117)
( 0.193266533, 0.0295116615)
( 0.194448898, 0.0300649197)
( 0.195631263, 0.0305913335)
( 0.196813627, 0.0310894069)
( 0.197995992, 0.031557711)
( 0.199178357, 0.0319948896)
( 0.200360721, 0.0323996636)
( 0.201543086, 0.032770836)
( 0.202725451, 0.0331072958)
( 0.203907816, 0.0334080223)
( 0.20509018, 0.0336720886)
( 0.206272545, 0.0338986655)
( 0.20745491, 0.0340870241)
( 0.208637275, 0.034236539)
( 0.209819639, 0.0343466904)
( 0.211002004, 0.0344170671)
( 0.212184369, 0.0344473673)
( 0.213366733, 0.0344374011)
( 0.214549098, 0.0343870911)
( 0.215731463, 0.0342964738)
( 0.216913828, 0.0341656995)
( 0.218096192, 0.033995033)
( 0.219278557, 0.0337848532)
( 0.220460922, 0.0335356525)
( 0.221643287, 0.0332480361)
( 0.222825651, 0.0329227205)
( 0.224008016, 0.0325605322)
( 0.225190381, 0.0321624051)
( 0.226372745, 0.0317293786)
( 0.22755511, 0.0312625945)
( 0.228737475, 0.0307632939)
( 0.22991984, 0.0302328134)
( 0.231102204, 0.0296725812)
( 0.232284569, 0.0290841127)
( 0.233466934, 0.0284690058)
( 0.234649299, 0.0278289352)
( 0.235831663, 0.0271656471)
( 0.237014028, 0.0264809531)
( 0.238196393, 0.025776724)
( 0.239378758, 0.0250548824)
( 0.240561122, 0.0243173963)
( 0.241743487, 0.023566271)
( 0.242925852, 0.0228035417)
( 0.244108216, 0.0220312652)
( 0.245290581, 0.0212515117)
( 0.246472946, 0.0204663558)
( 0.247655311, 0.0196778684)
( 0.248837675, 0.0188881072)
( 0.25002004, 0.018099108)
( 0.251202405, 0.0173128756)
( 0.25238477, 0.0165313745)
( 0.253567134, 0.0157565204)
( 0.254749499, 0.0149901709)
( 0.255931864, 0.014234117)
( 0.257114228, 0.0134900748)
( 0.258296593, 0.0127596777)
( 0.259478958, 0.0120444682)
( 0.260661323, 0.0113458913)
( 0.261843687, 0.0106652877)
( 0.263026052, 0.0100038878)
( 0.264208417, 0.0093628068)
( 0.265390782, 0.00874303987)
( 0.266573146, 0.00814545866)
( 0.267755511, 0.00757080851)
( 0.268937876, 0.00701970655)
( 0.27012024, 0.00649264082)
( 0.271302605, 0.00598997031)
( 0.27248497, 0.00551192602)
( 0.273667335, 0.00505861304)
( 0.274849699, 0.00463001351)
( 0.276032064, 0.00422599071)
( 0.277214429, 0.0038462939)
( 0.278396794, 0.00349056415)
( 0.279579158, 0.00315834097)
( 0.280761523, 0.00284906961)
( 0.281943888, 0.0025621091)
( 0.283126253, 0.00229674081)
( 0.284308617, 0.00205217745)
( 0.285490982, 0.0018275724)
( 0.286673347, 0.00162202931)
( 0.287855711, 0.00143461175)
( 0.289038076, 0.00126435287)
( 0.290220441, 0.00111026485)
( 0.291402806, 0.000971348198)
( 0.29258517, 0.000846600574)
( 0.293767535, 0.000735025189)
( 0.2949499, 0.000635638622)
( 0.296132265, 0.000547477992)
( 0.297314629, 0.000469607413)
( 0.298496994, 0.000401123685)
( 0.299679359, 0.000341161179)
( 0.300861723, 0.000288895903)
( 0.302044088, 0.000243548738)
( 0.303226453, 0.000204387855)
( 0.304408818, 0.000170730352)
( 0.305591182, 0.000141943126)
( 0.306773547, 0.00011744305)
( 0.307955912, 9.66965118e-5)
( 0.309138277, 7.92183691e-5)
( 0.310320641, 6.4570415e-5)
( 0.311503006, 5.23594139e-5)
( 0.312685371, 4.22347954e-5)
( 0.313867735, 3.38860809e-5)
( 0.3150501, 2.70401172e-5)
( 0.316232465, 2.14581907e-5)
( 0.31741483, 1.69330843e-5)
( 0.318597194, 1.32861379e-5)
( 0.319779559, 1.0364363e-5)
( 0.320961924, 8.03765429e-6)
( 0.322144289, 6.19613396e-6)
( 0.323326653, 4.74765607e-6)
( 0.324509018, 3.61549033e-6)
( 0.325691383, 2.73619813e-6)
( 0.326873747, 2.057707e-6)
( 0.328056112, 1.53758409e-6)
( 0.329238477, 1.14150474e-6)
( 0.330420842, 8.41908129e-7)
( 0.331603206, 6.16829304e-7)
( 0.332785571, 4.4889454e-7)
( 0.333967936, 3.24465844e-7)
( 0.335150301, 2.32919534e-7)
( 0.336332665, 1.66043803e-7)
( 0.33751503, 1.17540493e-7)
( 0.338697395, 8.26169902e-8)
( 0.33987976, 5.76551268e-8)
( 0.341062124, 3.994511e-8)
( 0.342244489, 2.74737313e-8)
( 0.343426854, 1.87573727e-8)
( 0.344609218, 1.27115799e-8)
( 0.345791583, 8.55015292e-9)
( 0.346973948, 5.70781099e-9)
( 0.348156313, 3.78148196e-9)
( 0.349338677, 2.4861511e-9)
( 0.350521042, 1.62197156e-9)
( 0.351703407, 1.04999515e-9)
( 0.352885772, 6.74432863e-10)
( 0.354068136, 4.29810978e-10)
( 0.355250501, 2.71759384e-10)
( 0.356432866, 1.70467552e-10)
( 0.35761523, 1.06079595e-10)
( 0.358797595, 6.54845292e-11)
( 0.35997996, 4.01002455e-11)
( 0.361162325, 2.43580497e-11)
( 0.362344689, 1.46761385e-11)
( 0.363527054, 8.77086656e-12)
( 0.364709419, 5.19904016e-12)
( 0.365891784, 3.05663302e-12)
( 0.367074148, 1.78235136e-12)
( 0.368256513, 1.03077669e-12)
( 0.369438878, 5.91220358e-13)
( 0.370621242, 3.36310845e-13)
( 0.371803607, 1.89728747e-13)
( 0.372985972, 1.06150277e-13)
( 0.374168337, 5.88980162e-14)
( 0.375350701, 3.24092076e-14)
( 0.376533066, 1.76856843e-14)
( 0.377715431, 9.57104473e-15)
( 0.378897796, 5.13664981e-15)
( 0.38008016, 2.73390611e-15)
( 0.381262525, 1.44301519e-15)
( 0.38244489, 7.55341362e-16)
( 0.383627255, 3.92105366e-16)
( 0.384809619, 2.01860924e-16)
( 0.385991984, 1.03061188e-16)
( 0.387174349, 5.21837835e-17)
( 0.388356713, 2.62046438e-17)
( 0.389539078, 1.30505429e-17)
( 0.390721443, 6.44603181e-18)
( 0.391903808, 3.15773976e-18)
( 0.393086172, 1.53421866e-18)
( 0.394268537, 7.3932049e-19)
( 0.395450902, 3.53362759e-19)
( 0.396633267, 1.67517362e-19)
( 0.397815631, 7.87696248e-20)
( 0.398997996, 3.67389665e-20)
( 0.400180361, 1.6997067e-20)
( 0.401362725, 7.80027619e-21)
( 0.40254509, 3.55095609e-21)
( 0.403727455, 1.60358007e-21)
( 0.40490982, 7.18384608e-22)
( 0.406092184, 3.19268199e-22)
( 0.407274549, 1.40766102e-22)
( 0.408456914, 6.15738077e-23)
( 0.409639279, 2.67215327e-23)
( 0.410821643, 1.15055199e-23)
( 0.412004008, 4.91521959e-24)
( 0.413186373, 2.08345338e-24)
( 0.414368737, 8.76276869e-25)
( 0.415551102, 3.65702741e-25)
( 0.416733467, 1.51445744e-25)
( 0.417915832, 6.22358551e-26)
( 0.419098196, 2.53800083e-26)
( 0.420280561, 1.0271247e-26)
( 0.421462926, 4.12522554e-27)
( 0.422645291, 1.64428892e-27)
( 0.423827655, 6.50469936e-28)
( 0.42501002, 2.55392246e-28)
( 0.426192385, 9.95250077e-29)
( 0.427374749, 3.84957994e-29)
( 0.428557114, 1.477963e-29)
( 0.429739479, 5.63242298e-30)
( 0.430921844, 2.13069215e-30)
( 0.432104208, 8.00114299e-31)
( 0.433286573, 2.98264271e-31)
( 0.434468938, 1.10377397e-31)
( 0.435651303, 4.05508957e-32)
( 0.436833667, 1.47901863e-32)
( 0.438016032, 5.35563592e-33)
( 0.439198397, 1.92541243e-33)
( 0.440380762, 6.8726264e-34)
( 0.441563126, 2.43567112e-34)
( 0.442745491, 8.57081233e-35)
( 0.443927856, 2.99462887e-35)
( 0.44511022, 1.03894302e-35)
( 0.446292585, 3.57913381e-36)
( 0.44747495, 1.22436568e-36)
( 0.448657315, 4.15911224e-37)
( 0.449839679, 1.40299277e-37)
( 0.451022044, 4.69985295e-38)
( 0.452204409, 1.56349189e-38)
( 0.453386774, 5.1653259e-39)
( 0.454569138, 1.69472206e-39)
( 0.455751503, 5.52211621e-40)
( 0.456933868, 1.78700706e-40)
( 0.458116232, 5.74338242e-41)
( 0.459298597, 1.83331344e-41)
( 0.460480962, 5.81218896e-42)
( 0.461663327, 1.8301342e-42)
( 0.462845691, 5.72363926e-43)
( 0.464028056, 1.77792436e-43)
( 0.465210421, 5.48543809e-44)
( 0.466392786, 1.68101414e-44)
( 0.46757515, 5.11679631e-45)
( 0.468757515, 1.54702027e-45)
( 0.46993988, 4.6458918e-46)
( 0.471122244, 1.38586582e-46)
( 0.472304609, 4.10634827e-47)
( 0.473486974, 1.20858186e-47)
( 0.474669339, 3.53333613e-48)
( 0.475851703, 1.02608897e-48)
( 0.477034068, 2.95991037e-49)
( 0.478216433, 8.48140054e-50)
( 0.479398798, 2.41409168e-50)
( 0.480581162, 6.82556361e-51)
( 0.481763527, 1.91700375e-51)
( 0.482945892, 5.34820325e-52)
( 0.484128257, 1.48215584e-52)
( 0.485310621, 4.08019663e-53)
( 0.486492986, 1.11575675e-53)
( 0.487675351, 3.03081074e-54)
( 0.488857715, 8.17802352e-55)
( 0.49004008, 2.19198325e-55)
( 0.491222445, 5.83612064e-56)
( 0.49240481, 1.54350479e-56)
( 0.493587174, 4.05496073e-57)
( 0.494769539, 1.05817687e-57)
( 0.495951904, 2.74296671e-58)
( 0.497134269, 7.06270251e-59)
( 0.498316633, 1.80636945e-59)
( 0.499498998, 4.58906757e-60)
( 0.500681363, 1.15803368e-60)
( 0.501863727, 2.90264008e-61)
( 0.503046092, 7.22664276e-62)
( 0.504228457, 1.78709349e-62)
( 0.505410822, 4.38955891e-63)
( 0.506593186, 1.07090956e-63)
( 0.507775551, 2.59500473e-64)
( 0.508957916, 6.24556666e-65)
( 0.510140281, 1.49296123e-65)
( 0.511322645, 3.54456223e-66)
( 0.51250501, 8.35811324e-67)
( 0.513687375, 1.95739918e-67)
( 0.514869739, 4.55270767e-68)
( 0.516052104, 1.05165383e-68)
( 0.517234469, 2.41258033e-69)
( 0.518416834, 5.49654392e-70)
( 0.519599198, 1.24362477e-70)
( 0.520781563, 2.79430197e-71)
( 0.521963928, 6.23496437e-72)
( 0.523146293, 1.38153984e-72)
( 0.524328657, 3.03985992e-73)
( 0.525511022, 6.64195841e-74)
( 0.526693387, 1.44106194e-74)
( 0.527875752, 3.10459062e-75)
( 0.529058116, 6.6412879e-76)
( 0.530240481, 1.41064396e-76)
( 0.531422846, 2.97502298e-77)
( 0.53260521, 6.22961918e-78)
( 0.533787575, 1.29515335e-78)
( 0.53496994, 2.67337246e-79)
( 0.536152305, 5.47855703e-80)
( 0.537334669, 1.11463072e-80)
( 0.538517034, 2.25135198e-81)
( 0.539699399, 4.51432305e-82)
( 0.540881764, 8.98602858e-83)
( 0.542064128, 1.77565165e-83)
( 0.543246493, 3.48298221e-84)
( 0.544428858, 6.78167173e-85)
( 0.545611222, 1.31069793e-85)
( 0.546793587, 2.51441485e-86)
( 0.547975952, 4.78770823e-87)
( 0.549158317, 9.04820849e-88)
( 0.550340681, 1.69718537e-88)
( 0.551523046, 3.15947635e-89)
( 0.552705411, 5.83723658e-90)
( 0.553887776, 1.0702688e-90)
( 0.55507014, 1.94741569e-91)
( 0.556252505, 3.51634398e-92)
( 0.55743487, 6.30053474e-93)
( 0.558617234, 1.12021953e-93)
( 0.559799599, 1.97630814e-94)
( 0.560981964, 3.45953644e-95)
( 0.562164329, 6.00867408e-96)
( 0.563346693, 1.03543408e-96)
( 0.564529058, 1.77025053e-97)
( 0.565711423, 3.00262227e-98)
( 0.566893788, 5.05248925e-99)
( 0.568076152, 8.43400174e-100)
( 0.569258517, 1.39659424e-100)
( 0.570440882, 2.29403257e-101)
( 0.571623246, 3.73771346e-102)
( 0.572805611, 6.04051077e-103)
( 0.573987976, 9.68247788e-104)
( 0.575170341, 1.53931795e-104)
( 0.576352705, 2.42707231e-105)
( 0.57753507, 3.79518608e-106)
( 0.578717435, 5.88521914e-107)
( 0.5798998, 9.05012247e-108)
( 0.581082164, 1.38003909e-108)
( 0.582264529, 2.08668122e-109)
( 0.583446894, 3.12846362e-110)
( 0.584629259, 4.65048977e-111)
( 0.585811623, 6.85395072e-112)
( 0.586993988, 1.00147448e-112)
( 0.588176353, 1.45069849e-113)
( 0.589358717, 2.08321617e-114)
( 0.590541082, 2.96546485e-115)
( 0.591723447, 4.18440437e-116)
( 0.592905812, 5.85245256e-117)
( 0.594088176, 8.11309045e-118)
( 0.595270541, 1.11470376e-118)
( 0.596452906, 1.51788099e-119)
( 0.597635271, 2.04833629e-120)
( 0.598817635, 2.73923981e-121)
( 0.6, 3.62997701e-122)
};
\addplot [red  ,dashed]
coordinates {
( 0.03, 0)
( 0.03755102, 0)
( 0.045102041, 0.0025)
( 0.052653061, 0.02)
( 0.060204082, 0.0275)
( 0.067755102, 0.085)
( 0.075306122, 0.2075)
( 0.082857143, 0.315)
( 0.090408163, 0.37)
( 0.097959184, 0.4625)
( 0.1055102, 0.495)
( 0.11306122, 0.4875)
( 0.12061224, 0.5)
( 0.12816327, 0.5025)
( 0.13571429, 0.4275)
( 0.14326531, 0.355)
( 0.15081633, 0.3225)
( 0.15836735, 0.21)
( 0.16591837, 0.125)
( 0.17346939, 0.035)
( 0.18102041, 0.015)
( 0.18857143, 0)
( 0.19612245, 0)
( 0.20367347, 0)
( 0.21122449, 0)
( 0.21877551, 0)
( 0.22632653, 0)
( 0.23387755, 0)
( 0.24142857, 0)
( 0.24897959, 0)
( 0.25653061, 0)
( 0.26408163, 0)
( 0.27163265, 0)
( 0.27918367, 0)
( 0.28673469, 0)
( 0.29428571, 0)
( 0.30183673, 0)
( 0.30938776, 0)
( 0.31693878, 0)
( 0.3244898, 0)
( 0.33204082, 0)
( 0.33959184, 0)
( 0.34714286, 0)
( 0.35469388, 0)
( 0.3622449, 0)
( 0.36979592, 0)
( 0.37734694, 0)
( 0.38489796, 0)
( 0.39244898, 0)
( 0.4, 0)
( 0.6, 0)
( 0.8, 0)
( 0.99, 0)
};
\addplot [red  ,dotted]
coordinates {
( 0.01, 5.58688753e-61)
( 0.0111823647, 2.10965406e-54)
( 0.0123647295, 9.23312948e-49)
( 0.0135470942, 7.08030114e-44)
( 0.0147294589, 1.29639765e-39)
( 0.0159118236, 7.18937063e-36)
( 0.0170941884, 1.45535903e-32)
( 0.0182765531, 1.24836544e-29)
( 0.0194589178, 5.12086381e-27)
( 0.0206412826, 1.10955943e-24)
( 0.0218236473, 1.37926135e-22)
( 0.023006012, 1.05425215e-20)
( 0.0241883768, 5.25449765e-19)
( 0.0253707415, 1.79530748e-17)
( 0.0265531062, 4.38954573e-16)
( 0.0277354709, 7.97030359e-15)
( 0.0289178357, 1.10987915e-13)
( 0.0301002004, 1.21898982e-12)
( 0.0312825651, 1.08219815e-11)
( 0.0324649299, 7.93522998e-11)
( 0.0336472946, 4.89792339e-10)
( 0.0348296593, 2.58798636e-9)
( 0.036012024, 1.18817515e-8)
( 0.0371943888, 4.80308692e-8)
( 0.0383767535, 1.72985362e-7)
( 0.0395591182, 5.60954672e-7)
( 0.040741483, 1.65339583e-6)
( 0.0419238477, 4.46720894e-6)
( 0.0431062124, 1.11484461e-5)
( 0.0442885772, 2.58756477e-5)
( 0.0454709419, 5.62026232e-5)
( 0.0466533066, 0.000114879425)
( 0.0478356713, 0.000222101146)
( 0.0490180361, 0.000408019075)
( 0.0502004008, 0.000715232121)
( 0.0513827655, 0.00120088901)
( 0.0525651303, 0.00193800116)
( 0.053747495, 0.00301560783)
( 0.0549298597, 0.00453754781)
( 0.0561122244, 0.00661975648)
( 0.0572945892, 0.00938619401)
( 0.0584769539, 0.012963685)
( 0.0596593186, 0.0174760842)
( 0.0608416834, 0.0230382549)
( 0.0620240481, 0.0297503561)
( 0.0632064128, 0.0376928778)
( 0.0643887776, 0.0469227685)
( 0.0655711423, 0.0574708696)
( 0.066753507, 0.0693407435)
( 0.0679358717, 0.0825088559)
( 0.0691182365, 0.0969259776)
( 0.0703006012, 0.112519596)
( 0.0714829659, 0.129197089)
( 0.0726653307, 0.146849396)
( 0.0738476954, 0.165354943)
( 0.0750300601, 0.184583586)
( 0.0762124248, 0.204400395)
( 0.0773947896, 0.224669133)
( 0.0785771543, 0.245255333)
( 0.079759519, 0.266028906)
( 0.0809418838, 0.286866259)
( 0.0821242485, 0.307651935)
( 0.0833066132, 0.328279788)
( 0.084488978, 0.348653734)
( 0.0856713427, 0.368688146)
( 0.0868537074, 0.388307918)
( 0.0880360721, 0.407448286)
( 0.0892184369, 0.426054436)
( 0.0904008016, 0.444080955)
( 0.0915831663, 0.461491177)
( 0.0927655311, 0.478256451)
( 0.0939478958, 0.494355378)
( 0.0951302605, 0.509773022)
( 0.0963126253, 0.524500138)
( 0.09749499, 0.538532427)
( 0.0986773547, 0.551869816)
( 0.0998597194, 0.564515793)
( 0.101042084, 0.576476786)
( 0.102224449, 0.587761597)
( 0.103406814, 0.598380885)
( 0.104589178, 0.608346708)
( 0.105771543, 0.617672106)
( 0.106953908, 0.626370743)
( 0.108136273, 0.634456578)
( 0.109318637, 0.641943591)
( 0.110501002, 0.648845537)
( 0.111683367, 0.655175738)
( 0.112865731, 0.660946897)
( 0.114048096, 0.666170947)
( 0.115230461, 0.670858913)
( 0.116412826, 0.675020803)
( 0.11759519, 0.678665509)
( 0.118777555, 0.681800722)
( 0.11995992, 0.684432865)
( 0.121142285, 0.686567026)
( 0.122324649, 0.688206912)
( 0.123507014, 0.689354798)
( 0.124689379, 0.69001149)
( 0.125871743, 0.690176292)
( 0.127054108, 0.68984697)
( 0.128236473, 0.689019738)
( 0.129418838, 0.687689226)
( 0.130601202, 0.685848476)
( 0.131783567, 0.683488924)
( 0.132965932, 0.680600408)
( 0.134148297, 0.677171168)
( 0.135330661, 0.673187871)
( 0.136513026, 0.668635641)
( 0.137695391, 0.663498112)
( 0.138877756, 0.657757495)
( 0.14006012, 0.651394681)
( 0.141242485, 0.644389364)
( 0.14242485, 0.636720209)
( 0.143607214, 0.628365055)
( 0.144789579, 0.619301182)
( 0.145971944, 0.609505621)
( 0.147154309, 0.598955551)
( 0.148336673, 0.587628752)
( 0.149519038, 0.575504167)
( 0.150701403, 0.562562547)
( 0.151883768, 0.548787201)
( 0.153066132, 0.534164869)
( 0.154248497, 0.518686698)
( 0.155430862, 0.502349348)
( 0.156613226, 0.485156207)
( 0.157795591, 0.467118709)
( 0.158977956, 0.448257739)
( 0.160160321, 0.428605091)
( 0.161342685, 0.40820494)
( 0.16252505, 0.38711527)
( 0.163707415, 0.365409175)
( 0.16488978, 0.343175954)
( 0.166072144, 0.320521887)
( 0.167254509, 0.297570561)
( 0.168436874, 0.274462619)
( 0.169619238, 0.251354793)
( 0.170801603, 0.228418093)
( 0.171983968, 0.205835037)
( 0.173166333, 0.183795862)
( 0.174348697, 0.162493716)
( 0.175531062, 0.142118883)
( 0.176713427, 0.122852246)
( 0.177895792, 0.104858254)
( 0.179078156, 0.0882777964)
( 0.180260521, 0.0732214963)
( 0.181442886, 0.0597639763)
( 0.182625251, 0.0479396894)
( 0.183807615, 0.0377408372)
( 0.18498998, 0.029117769)
( 0.186172345, 0.0219820403)
( 0.187354709, 0.0162120315)
( 0.188537074, 0.0116607287)
( 0.189719439, 0.00816498418)
( 0.190901804, 0.00555536829)
( 0.192084168, 0.00366563642)
( 0.193266533, 0.00234089555)
( 0.194448898, 0.00144376124)
( 0.195631263, 0.000858110844)
( 0.196813627, 0.000490401414)
( 0.197995992, 0.000268856351)
( 0.199178357, 0.000141067313)
( 0.200360721, 7.06688214e-5)
( 0.201543086, 3.37183839e-5)
( 0.202725451, 1.5285278e-5)
( 0.203907816, 6.5670478e-6)
( 0.20509018, 2.66732845e-6)
( 0.206272545, 1.02167502e-6)
( 0.20745491, 3.68133534e-7)
( 0.208637275, 1.24477628e-7)
( 0.209819639, 3.94024232e-8)
( 0.211002004, 1.16485735e-8)
( 0.212184369, 3.20876544e-9)
( 0.213366733, 8.21760151e-10)
( 0.214549098, 1.95233383e-10)
( 0.215731463, 4.29400585e-11)
( 0.216913828, 8.72589194e-12)
( 0.218096192, 1.63523327e-12)
( 0.219278557, 2.82100868e-13)
( 0.220460922, 4.47267128e-14)
( 0.221643287, 6.50734306e-15)
( 0.222825651, 8.6757332e-16)
( 0.224008016, 1.05857811e-16)
( 0.225190381, 1.18075659e-17)
( 0.226372745, 1.20277371e-18)
( 0.22755511, 1.11793885e-19)
( 0.228737475, 9.47428355e-21)
( 0.22991984, 7.31663336e-22)
( 0.231102204, 5.14651402e-23)
( 0.232284569, 3.2961674e-24)
( 0.233466934, 1.92181865e-25)
( 0.234649299, 1.01997442e-26)
( 0.235831663, 4.92786227e-28)
( 0.237014028, 2.16764817e-29)
( 0.238196393, 8.68352579e-31)
( 0.239378758, 3.16914222e-32)
( 0.240561122, 1.05421574e-33)
( 0.241743487, 3.19818144e-35)
( 0.242925852, 8.85407894e-37)
( 0.244108216, 2.23854379e-38)
( 0.245290581, 5.17269071e-40)
( 0.246472946, 1.09338148e-41)
( 0.247655311, 2.11608334e-43)
( 0.248837675, 3.75339714e-45)
( 0.25002004, 6.10790664e-47)
( 0.251202405, 9.12850777e-49)
( 0.25238477, 1.25436978e-50)
( 0.253567134, 1.58657884e-52)
( 0.254749499, 1.8493138e-54)
( 0.255931864, 1.98876517e-56)
( 0.257114228, 1.97559438e-58)
( 0.258296593, 1.81499429e-60)
( 0.259478958, 1.54397506e-62)
( 0.260661323, 1.21763729e-64)
( 0.261843687, 8.91317596e-67)
( 0.263026052, 6.06325424e-69)
( 0.264208417, 3.83756693e-71)
( 0.265390782, 2.26253932e-73)
( 0.266573146, 1.24403679e-75)
( 0.267755511, 6.38655914e-78)
( 0.268937876, 3.06470601e-80)
( 0.27012024, 1.37619956e-82)
( 0.271302605, 5.78918635e-85)
( 0.27248497, 2.28380797e-87)
( 0.273667335, 8.45783189e-90)
( 0.274849699, 2.94344533e-92)
( 0.276032064, 9.63559602e-95)
( 0.277214429, 2.9699077e-97)
( 0.278396794, 8.62685991e-100)
( 0.279579158, 2.36373629e-102)
( 0.280761523, 6.11448801e-105)
( 0.281943888, 1.49451907e-107)
( 0.283126253, 3.45442472e-110)
( 0.284308617, 7.55653482e-113)
( 0.285490982, 1.56555847e-115)
( 0.286673347, 3.07418357e-118)
( 0.287855711, 5.72540032e-121)
( 0.289038076, 1.01201439e-123)
( 0.290220441, 1.69882727e-126)
( 0.291402806, 2.70993167e-129)
( 0.29258517, 4.11023886e-132)
( 0.293767535, 5.93084803e-135)
( 0.2949499, 8.14587232e-138)
( 0.296132265, 1.06548767e-140)
( 0.297314629, 1.32787569e-143)
( 0.298496994, 1.57747393e-146)
( 0.299679359, 1.78710511e-149)
( 0.300861723, 1.93151711e-152)
( 0.302044088, 1.99239459e-155)
( 0.303226453, 1.96218024e-158)
( 0.304408818, 1.84560424e-161)
( 0.305591182, 1.65849832e-164)
( 0.306773547, 1.42429669e-167)
( 0.307955912, 1.16928107e-170)
( 0.309138277, 9.17881465e-174)
( 0.310320641, 6.8914745e-177)
( 0.311503006, 4.94990597e-180)
( 0.312685371, 3.40200826e-183)
( 0.313867735, 2.23776799e-186)
( 0.3150501, 1.40902027e-189)
( 0.316232465, 8.4940915e-193)
( 0.31741483, 4.90324097e-196)
( 0.318597194, 2.71068816e-199)
( 0.319779559, 1.43537002e-202)
( 0.320961924, 7.28096497e-206)
( 0.322144289, 3.53836441e-209)
( 0.323326653, 1.6475847e-212)
( 0.324509018, 7.35128069e-216)
( 0.325691383, 3.1432756e-219)
( 0.326873747, 1.28806007e-222)
( 0.328056112, 5.05882922e-226)
( 0.329238477, 1.90434853e-229)
( 0.330420842, 6.87138126e-233)
( 0.331603206, 2.37661098e-236)
( 0.332785571, 7.87953476e-240)
( 0.333967936, 2.50426538e-243)
( 0.335150301, 7.62962738e-247)
( 0.336332665, 2.22829455e-250)
( 0.33751503, 6.23862033e-254)
( 0.338697395, 1.67436082e-257)
( 0.33987976, 4.30774002e-261)
( 0.341062124, 1.06238749e-264)
( 0.342244489, 2.51154128e-268)
( 0.343426854, 5.69128581e-272)
( 0.344609218, 1.23617498e-275)
( 0.345791583, 2.57355744e-279)
( 0.346973948, 5.13517455e-283)
( 0.348156313, 9.820313e-287)
( 0.349338677, 1.79979864e-290)
( 0.350521042, 3.16103358e-294)
( 0.351703407, 5.32007222e-298)
( 0.352885772, 8.57954786e-302)
( 0.354068136, 1.32569486e-305)
( 0.355250501, 1.96258095e-309)
( 0.356432866, 2.78347769e-313)
( 0.35761523, 3.78176225e-317)
( 0.358797595, 4.92089383e-321)
( 0.35997996, 0)
( 0.361162325, 0)
( 0.362344689, 0)
( 0.363527054, 0)
( 0.364709419, 0)
( 0.365891784, 0)
( 0.367074148, 0)
( 0.368256513, 0)
( 0.369438878, 0)
( 0.370621242, 0)
( 0.371803607, 0)
( 0.372985972, 0)
( 0.374168337, 0)
( 0.375350701, 0)
( 0.376533066, 0)
( 0.377715431, 0)
( 0.378897796, 0)
( 0.38008016, 0)
( 0.381262525, 0)
( 0.38244489, 0)
( 0.383627255, 0)
( 0.384809619, 0)
( 0.385991984, 0)
( 0.387174349, 0)
( 0.388356713, 0)
( 0.389539078, 0)
( 0.390721443, 0)
( 0.391903808, 0)
( 0.393086172, 0)
( 0.394268537, 0)
( 0.395450902, 0)
( 0.396633267, 0)
( 0.397815631, 0)
( 0.398997996, 0)
( 0.400180361, 0)
( 0.401362725, 0)
( 0.40254509, 0)
( 0.403727455, 0)
( 0.40490982, 0)
( 0.406092184, 0)
( 0.407274549, 0)
( 0.408456914, 0)
( 0.409639279, 0)
( 0.410821643, 0)
( 0.412004008, 0)
( 0.413186373, 0)
( 0.414368737, 0)
( 0.415551102, 0)
( 0.416733467, 0)
( 0.417915832, 0)
( 0.419098196, 0)
( 0.420280561, 0)
( 0.421462926, 0)
( 0.422645291, 0)
( 0.423827655, 0)
( 0.42501002, 0)
( 0.426192385, 0)
( 0.427374749, 0)
( 0.428557114, 0)
( 0.429739479, 0)
( 0.430921844, 0)
( 0.432104208, 0)
( 0.433286573, 0)
( 0.434468938, 0)
( 0.435651303, 0)
( 0.436833667, 0)
( 0.438016032, 0)
( 0.439198397, 0)
( 0.440380762, 0)
( 0.441563126, 0)
( 0.442745491, 0)
( 0.443927856, 0)
( 0.44511022, 0)
( 0.446292585, 0)
( 0.44747495, 0)
( 0.448657315, 0)
( 0.449839679, 0)
( 0.451022044, 0)
( 0.452204409, 0)
( 0.453386774, 0)
( 0.454569138, 0)
( 0.455751503, 0)
( 0.456933868, 0)
( 0.458116232, 0)
( 0.459298597, 0)
( 0.460480962, 0)
( 0.461663327, 0)
( 0.462845691, 0)
( 0.464028056, 0)
( 0.465210421, 0)
( 0.466392786, 0)
( 0.46757515, 0)
( 0.468757515, 0)
( 0.46993988, 0)
( 0.471122244, 0)
( 0.472304609, 0)
( 0.473486974, 0)
( 0.474669339, 0)
( 0.475851703, 0)
( 0.477034068, 0)
( 0.478216433, 0)
( 0.479398798, 0)
( 0.480581162, 0)
( 0.481763527, 0)
( 0.482945892, 0)
( 0.484128257, 0)
( 0.485310621, 0)
( 0.486492986, 0)
( 0.487675351, 0)
( 0.488857715, 0)
( 0.49004008, 0)
( 0.491222445, 0)
( 0.49240481, 0)
( 0.493587174, 0)
( 0.494769539, 0)
( 0.495951904, 0)
( 0.497134269, 0)
( 0.498316633, 0)
( 0.499498998, 0)
( 0.500681363, 0)
( 0.501863727, 0)
( 0.503046092, 0)
( 0.504228457, 0)
( 0.505410822, 0)
( 0.506593186, 0)
( 0.507775551, 0)
( 0.508957916, 0)
( 0.510140281, 0)
( 0.511322645, 0)
( 0.51250501, 0)
( 0.513687375, 0)
( 0.514869739, 0)
( 0.516052104, 0)
( 0.517234469, 0)
( 0.518416834, 0)
( 0.519599198, 0)
( 0.520781563, 0)
( 0.521963928, 0)
( 0.523146293, 0)
( 0.524328657, 0)
( 0.525511022, 0)
( 0.526693387, 0)
( 0.527875752, 0)
( 0.529058116, 0)
( 0.530240481, 0)
( 0.531422846, 0)
( 0.53260521, 0)
( 0.533787575, 0)
( 0.53496994, 0)
( 0.536152305, 0)
( 0.537334669, 0)
( 0.538517034, 0)
( 0.539699399, 0)
( 0.540881764, 0)
( 0.542064128, 0)
( 0.543246493, 0)
( 0.544428858, 0)
( 0.545611222, 0)
( 0.546793587, 0)
( 0.547975952, 0)
( 0.549158317, 0)
( 0.550340681, 0)
( 0.551523046, 0)
( 0.552705411, 0)
( 0.553887776, 0)
( 0.55507014, 0)
( 0.556252505, 0)
( 0.55743487, 0)
( 0.558617234, 0)
( 0.559799599, 0)
( 0.560981964, 0)
( 0.562164329, 0)
( 0.563346693, 0)
( 0.564529058, 0)
( 0.565711423, 0)
( 0.566893788, 0)
( 0.568076152, 0)
( 0.569258517, 0)
( 0.570440882, 0)
( 0.571623246, 0)
( 0.572805611, 0)
( 0.573987976, 0)
( 0.575170341, 0)
( 0.576352705, 0)
( 0.57753507, 0)
( 0.578717435, 0)
( 0.5798998, 0)
( 0.581082164, 0)
( 0.582264529, 0)
( 0.583446894, 0)
( 0.584629259, 0)
( 0.585811623, 0)
( 0.586993988, 0)
( 0.588176353, 0)
( 0.589358717, 0)
( 0.590541082, 0)
( 0.591723447, 0)
( 0.592905812, 0)
( 0.594088176, 0)
( 0.595270541, 0)
( 0.596452906, 0)
( 0.597635271, 0)
( 0.598817635, 0)
( 0.6, 0)
};
\addplot [gray ,]
coordinates {
( 0.019, 0)
( 0.023714286, 0.0975)
( 0.028428571, 0.4225)
( 0.033142857, 0.725)
( 0.037857143, 0.8975)
( 0.042571429, 0.945)
( 0.047285714, 0.975)
( 0.052, 0.985)
( 0.056714286, 1)
( 0.061428571, 0.995)
( 0.066142857, 0.9975)
( 0.070857143, 0.995)
( 0.075571429, 0.9975)
( 0.080285714, 0.995)
( 0.085, 0.99)
( 0.089714286, 0.985)
( 0.094428571, 0.9775)
( 0.099142857, 0.9675)
( 0.10385714, 0.8825)
( 0.10857143, 0.7125)
( 0.11328571, 0.445)
( 0.118, 0.1025)
( 0.12271429, 0.02)
( 0.12742857, 0)
( 0.13214286, 0)
( 0.13685714, 0)
( 0.14157143, 0)
( 0.14628571, 0)
( 0.151, 0)
( 0.15571429, 0)
( 0.16042857, 0)
( 0.16514286, 0)
( 0.16985714, 0)
( 0.17457143, 0)
( 0.17928571, 0)
( 0.184, 0)
( 0.18871429, 0)
( 0.19342857, 0)
( 0.19814286, 0)
( 0.20285714, 0)
( 0.20757143, 0)
( 0.21228571, 0)
( 0.217, 0)
( 0.22171429, 0)
( 0.22642857, 0)
( 0.23114286, 0)
( 0.23585714, 0)
( 0.24057143, 0)
( 0.24528571, 0)
( 0.25, 0)
( 0.3, 0)
( 0.6, 0)
( 0.99, 0)
};
\addplot [gray ,dotted]
coordinates {
( 0.01, 1.0102277e-29)
( 0.0111823647, 2.0701463e-22)
( 0.0123647295, 5.36471807e-17)
( 0.0135470942, 5.74097752e-13)
( 0.0147294589, 5.89315001e-10)
( 0.0159118236, 1.06674071e-7)
( 0.0170941884, 5.31039816e-6)
( 0.0182765531, 0.000100812063)
( 0.0194589178, 0.000929489623)
( 0.0206412826, 0.00498186921)
( 0.0218236473, 0.0177503645)
( 0.023006012, 0.0464829092)
( 0.0241883768, 0.0964669676)
( 0.0253707415, 0.167913213)
( 0.0265531062, 0.255841256)
( 0.0277354709, 0.352408415)
( 0.0289178357, 0.44967876)
( 0.0301002004, 0.541442159)
( 0.0312825651, 0.623825567)
( 0.0324649299, 0.695077485)
( 0.0336472946, 0.75500095)
( 0.0348296593, 0.80435781)
( 0.036012024, 0.8443921)
( 0.0371943888, 0.876505401)
( 0.0383767535, 0.902063141)
( 0.0395591182, 0.92229536)
( 0.040741483, 0.938258028)
( 0.0419238477, 0.950829365)
( 0.0431062124, 0.960724091)
( 0.0442885772, 0.968515149)
( 0.0454709419, 0.974657006)
( 0.0466533066, 0.979507523)
( 0.0478356713, 0.983347103)
( 0.0490180361, 0.98639476)
( 0.0502004008, 0.988821255)
( 0.0513827655, 0.990759623)
( 0.0525651303, 0.992313518)
( 0.053747495, 0.993563759)
( 0.0549298597, 0.994573439)
( 0.0561122244, 0.995391894)
( 0.0572945892, 0.996057779)
( 0.0584769539, 0.996601446)
( 0.0596593186, 0.997046783)
( 0.0608416834, 0.997412636)
( 0.0620240481, 0.997713907)
( 0.0632064128, 0.997962404)
( 0.0643887776, 0.998167498)
( 0.0655711423, 0.998336634)
( 0.066753507, 0.998475727)
( 0.0679358717, 0.99858946)
( 0.0691182365, 0.998681531)
( 0.0703006012, 0.998754824)
( 0.0714829659, 0.99881155)
( 0.0726653307, 0.99885335)
( 0.0738476954, 0.998881364)
( 0.0750300601, 0.99889628)
( 0.0762124248, 0.998898356)
( 0.0773947896, 0.998887425)
( 0.0785771543, 0.998862868)
( 0.079759519, 0.99882357)
( 0.0809418838, 0.998767845)
( 0.0821242485, 0.998693318)
( 0.0833066132, 0.998596768)
( 0.084488978, 0.99847391)
( 0.0856713427, 0.998319087)
( 0.0868537074, 0.998124867)
( 0.0880360721, 0.997881486)
( 0.0892184369, 0.997576096)
( 0.0904008016, 0.997191742)
( 0.0915831663, 0.99670597)
( 0.0927655311, 0.996088928)
( 0.0939478958, 0.995300775)
( 0.0951302605, 0.994288148)
( 0.0963126253, 0.992979332)
( 0.09749499, 0.991277697)
( 0.0986773547, 0.989052797)
( 0.0998597194, 0.986128379)
( 0.101042084, 0.982266388)
( 0.102224449, 0.977145949)
( 0.103406814, 0.970336301)
( 0.104589178, 0.961263056)
( 0.105771543, 0.949168161)
( 0.106953908, 0.933066212)
( 0.108136273, 0.911704133)
( 0.109318637, 0.883538766)
( 0.110501002, 0.846758781)
( 0.111683367, 0.799393165)
( 0.112865731, 0.739564855)
( 0.114048096, 0.665952717)
( 0.115230461, 0.578493083)
( 0.116412826, 0.479246072)
( 0.11759519, 0.373144841)
( 0.118777555, 0.268086172)
( 0.11995992, 0.173723113)
( 0.121142285, 0.0987533428)
( 0.122324649, 0.0476271054)
( 0.123507014, 0.0187345057)
( 0.124689379, 0.00574196115)
( 0.125871743, 0.0013016949)
( 0.127054108, 0.000205949266)
( 0.128236473, 2.13404694e-5)
( 0.129418838, 1.35281065e-6)
( 0.130601202, 4.88400086e-8)
( 0.131783567, 9.32984977e-10)
( 0.132965932, 8.75826041e-12)
( 0.134148297, 3.75702999e-14)
( 0.135330661, 6.86860525e-17)
( 0.136513026, 5.01360331e-20)
( 0.137695391, 1.37685731e-23)
( 0.138877756, 1.34993152e-27)
( 0.14006012, 4.51892496e-32)
( 0.141242485, 4.98082593e-37)
( 0.14242485, 1.75827259e-42)
( 0.143607214, 1.95024503e-48)
( 0.144789579, 6.72389143e-55)
( 0.145971944, 7.18462069e-62)
( 0.147154309, 2.3895172e-69)
( 0.148336673, 2.50062364e-77)
( 0.149519038, 8.37189461e-86)
( 0.150701403, 9.16187998e-95)
( 0.151883768, 3.362542e-104)
( 0.153066132, 4.26044519e-114)
( 0.154248497, 1.92330521e-124)
( 0.155430862, 3.19866249e-135)
( 0.156613226, 2.0290052e-146)
( 0.157795591, 5.08585381e-158)
( 0.158977956, 5.22004068e-170)
( 0.160160321, 2.27293274e-182)
( 0.161342685, 4.34742811e-195)
( 0.16252505, 3.77896516e-208)
( 0.163707415, 1.54276376e-221)
( 0.16488978, 3.05319463e-235)
( 0.166072144, 3.01906607e-249)
( 0.167254509, 1.5351079e-263)
( 0.168436874, 4.12441631e-278)
( 0.169619238, 6.00707236e-293)
( 0.170801603, 4.85810493e-308)
( 0.171983968, 2.47032823e-323)
( 0.173166333, 0)
( 0.174348697, 0)
( 0.175531062, 0)
( 0.176713427, 0)
( 0.177895792, 0)
( 0.179078156, 0)
( 0.180260521, 0)
( 0.181442886, 0)
( 0.182625251, 0)
( 0.183807615, 0)
( 0.18498998, 0)
( 0.186172345, 0)
( 0.187354709, 0)
( 0.188537074, 0)
( 0.189719439, 0)
( 0.190901804, 0)
( 0.192084168, 0)
( 0.193266533, 0)
( 0.194448898, 0)
( 0.195631263, 0)
( 0.196813627, 0)
( 0.197995992, 0)
( 0.199178357, 0)
( 0.200360721, 0)
( 0.201543086, 0)
( 0.202725451, 0)
( 0.203907816, 0)
( 0.20509018, 0)
( 0.206272545, 0)
( 0.20745491, 0)
( 0.208637275, 0)
( 0.209819639, 0)
( 0.211002004, 0)
( 0.212184369, 0)
( 0.213366733, 0)
( 0.214549098, 0)
( 0.215731463, 0)
( 0.216913828, 0)
( 0.218096192, 0)
( 0.219278557, 0)
( 0.220460922, 0)
( 0.221643287, 0)
( 0.222825651, 0)
( 0.224008016, 0)
( 0.225190381, 0)
( 0.226372745, 0)
( 0.22755511, 0)
( 0.228737475, 0)
( 0.22991984, 0)
( 0.231102204, 0)
( 0.232284569, 0)
( 0.233466934, 0)
( 0.234649299, 0)
( 0.235831663, 0)
( 0.237014028, 0)
( 0.238196393, 0)
( 0.239378758, 0)
( 0.240561122, 0)
( 0.241743487, 0)
( 0.242925852, 0)
( 0.244108216, 0)
( 0.245290581, 0)
( 0.246472946, 0)
( 0.247655311, 0)
( 0.248837675, 0)
( 0.25002004, 0)
( 0.251202405, 0)
( 0.25238477, 0)
( 0.253567134, 0)
( 0.254749499, 0)
( 0.255931864, 0)
( 0.257114228, 0)
( 0.258296593, 0)
( 0.259478958, 0)
( 0.260661323, 0)
( 0.261843687, 0)
( 0.263026052, 0)
( 0.264208417, 0)
( 0.265390782, 0)
( 0.266573146, 0)
( 0.267755511, 0)
( 0.268937876, 0)
( 0.27012024, 0)
( 0.271302605, 0)
( 0.27248497, 0)
( 0.273667335, 0)
( 0.274849699, 0)
( 0.276032064, 0)
( 0.277214429, 0)
( 0.278396794, 0)
( 0.279579158, 0)
( 0.280761523, 0)
( 0.281943888, 0)
( 0.283126253, 0)
( 0.284308617, 0)
( 0.285490982, 0)
( 0.286673347, 0)
( 0.287855711, 0)
( 0.289038076, 0)
( 0.290220441, 0)
( 0.291402806, 0)
( 0.29258517, 0)
( 0.293767535, 0)
( 0.2949499, 0)
( 0.296132265, 0)
( 0.297314629, 0)
( 0.298496994, 0)
( 0.299679359, 0)
( 0.300861723, 0)
( 0.302044088, 0)
( 0.303226453, 0)
( 0.304408818, 0)
( 0.305591182, 0)
( 0.306773547, 0)
( 0.307955912, 0)
( 0.309138277, 0)
( 0.310320641, 0)
( 0.311503006, 0)
( 0.312685371, 0)
( 0.313867735, 0)
( 0.3150501, 0)
( 0.316232465, 0)
( 0.31741483, 0)
( 0.318597194, 0)
( 0.319779559, 0)
( 0.320961924, 0)
( 0.322144289, 0)
( 0.323326653, 0)
( 0.324509018, 0)
( 0.325691383, 0)
( 0.326873747, 0)
( 0.328056112, 0)
( 0.329238477, 0)
( 0.330420842, 0)
( 0.331603206, 0)
( 0.332785571, 0)
( 0.333967936, 0)
( 0.335150301, 0)
( 0.336332665, 0)
( 0.33751503, 0)
( 0.338697395, 0)
( 0.33987976, 0)
( 0.341062124, 0)
( 0.342244489, 0)
( 0.343426854, 0)
( 0.344609218, 0)
( 0.345791583, 0)
( 0.346973948, 0)
( 0.348156313, 0)
( 0.349338677, 0)
( 0.350521042, 0)
( 0.351703407, 0)
( 0.352885772, 0)
( 0.354068136, 0)
( 0.355250501, 0)
( 0.356432866, 0)
( 0.35761523, 0)
( 0.358797595, 0)
( 0.35997996, 0)
( 0.361162325, 0)
( 0.362344689, 0)
( 0.363527054, 0)
( 0.364709419, 0)
( 0.365891784, 0)
( 0.367074148, 0)
( 0.368256513, 0)
( 0.369438878, 0)
( 0.370621242, 0)
( 0.371803607, 0)
( 0.372985972, 0)
( 0.374168337, 0)
( 0.375350701, 0)
( 0.376533066, 0)
( 0.377715431, 0)
( 0.378897796, 0)
( 0.38008016, 0)
( 0.381262525, 0)
( 0.38244489, 0)
( 0.383627255, 0)
( 0.384809619, 0)
( 0.385991984, 0)
( 0.387174349, 0)
( 0.388356713, 0)
( 0.389539078, 0)
( 0.390721443, 0)
( 0.391903808, 0)
( 0.393086172, 0)
( 0.394268537, 0)
( 0.395450902, 0)
( 0.396633267, 0)
( 0.397815631, 0)
( 0.398997996, 0)
( 0.400180361, 0)
( 0.401362725, 0)
( 0.40254509, 0)
( 0.403727455, 0)
( 0.40490982, 0)
( 0.406092184, 0)
( 0.407274549, 0)
( 0.408456914, 0)
( 0.409639279, 0)
( 0.410821643, 0)
( 0.412004008, 0)
( 0.413186373, 0)
( 0.414368737, 0)
( 0.415551102, 0)
( 0.416733467, 0)
( 0.417915832, 0)
( 0.419098196, 0)
( 0.420280561, 0)
( 0.421462926, 0)
( 0.422645291, 0)
( 0.423827655, 0)
( 0.42501002, 0)
( 0.426192385, 0)
( 0.427374749, 0)
( 0.428557114, 0)
( 0.429739479, 0)
( 0.430921844, 0)
( 0.432104208, 0)
( 0.433286573, 0)
( 0.434468938, 0)
( 0.435651303, 0)
( 0.436833667, 0)
( 0.438016032, 0)
( 0.439198397, 0)
( 0.440380762, 0)
( 0.441563126, 0)
( 0.442745491, 0)
( 0.443927856, 0)
( 0.44511022, 0)
( 0.446292585, 0)
( 0.44747495, 0)
( 0.448657315, 0)
( 0.449839679, 0)
( 0.451022044, 0)
( 0.452204409, 0)
( 0.453386774, 0)
( 0.454569138, 0)
( 0.455751503, 0)
( 0.456933868, 0)
( 0.458116232, 0)
( 0.459298597, 0)
( 0.460480962, 0)
( 0.461663327, 0)
( 0.462845691, 0)
( 0.464028056, 0)
( 0.465210421, 0)
( 0.466392786, 0)
( 0.46757515, 0)
( 0.468757515, 0)
( 0.46993988, 0)
( 0.471122244, 0)
( 0.472304609, 0)
( 0.473486974, 0)
( 0.474669339, 0)
( 0.475851703, 0)
( 0.477034068, 0)
( 0.478216433, 0)
( 0.479398798, 0)
( 0.480581162, 0)
( 0.481763527, 0)
( 0.482945892, 0)
( 0.484128257, 0)
( 0.485310621, 0)
( 0.486492986, 0)
( 0.487675351, 0)
( 0.488857715, 0)
( 0.49004008, 0)
( 0.491222445, 0)
( 0.49240481, 0)
( 0.493587174, 0)
( 0.494769539, 0)
( 0.495951904, 0)
( 0.497134269, 0)
( 0.498316633, 0)
( 0.499498998, 0)
( 0.500681363, 0)
( 0.501863727, 0)
( 0.503046092, 0)
( 0.504228457, 0)
( 0.505410822, 0)
( 0.506593186, 0)
( 0.507775551, 0)
( 0.508957916, 0)
( 0.510140281, 0)
( 0.511322645, 0)
( 0.51250501, 0)
( 0.513687375, 0)
( 0.514869739, 0)
( 0.516052104, 0)
( 0.517234469, 0)
( 0.518416834, 0)
( 0.519599198, 0)
( 0.520781563, 0)
( 0.521963928, 0)
( 0.523146293, 0)
( 0.524328657, 0)
( 0.525511022, 0)
( 0.526693387, 0)
( 0.527875752, 0)
( 0.529058116, 0)
( 0.530240481, 0)
( 0.531422846, 0)
( 0.53260521, 0)
( 0.533787575, 0)
( 0.53496994, 0)
( 0.536152305, 0)
( 0.537334669, 0)
( 0.538517034, 0)
( 0.539699399, 0)
( 0.540881764, 0)
( 0.542064128, 0)
( 0.543246493, 0)
( 0.544428858, 0)
( 0.545611222, 0)
( 0.546793587, 0)
( 0.547975952, 0)
( 0.549158317, 0)
( 0.550340681, 0)
( 0.551523046, 0)
( 0.552705411, 0)
( 0.553887776, 0)
( 0.55507014, 0)
( 0.556252505, 0)
( 0.55743487, 0)
( 0.558617234, 0)
( 0.559799599, 0)
( 0.560981964, 0)
( 0.562164329, 0)
( 0.563346693, 0)
( 0.564529058, 0)
( 0.565711423, 0)
( 0.566893788, 0)
( 0.568076152, 0)
( 0.569258517, 0)
( 0.570440882, 0)
( 0.571623246, 0)
( 0.572805611, 0)
( 0.573987976, 0)
( 0.575170341, 0)
( 0.576352705, 0)
( 0.57753507, 0)
( 0.578717435, 0)
( 0.5798998, 0)
( 0.581082164, 0)
( 0.582264529, 0)
( 0.583446894, 0)
( 0.584629259, 0)
( 0.585811623, 0)
( 0.586993988, 0)
( 0.588176353, 0)
( 0.589358717, 0)
( 0.590541082, 0)
( 0.591723447, 0)
( 0.592905812, 0)
( 0.594088176, 0)
( 0.595270541, 0)
( 0.596452906, 0)
( 0.597635271, 0)
( 0.598817635, 0)
( 0.6, 0)
};
\addplot [blue ,dashed]
coordinates {
( 0.01, 0.5075)
( 0.013877551, 0.975)
( 0.017755102, 1)
( 0.021632653, 1)
( 0.025510204, 1)
( 0.029387755, 1)
( 0.033265306, 1)
( 0.037142857, 1)
( 0.041020408, 1)
( 0.044897959, 1)
( 0.04877551, 1)
( 0.052653061, 1)
( 0.056530612, 1)
( 0.060408163, 1)
( 0.064285714, 1)
( 0.068163265, 0.9975)
( 0.072040816, 0.9)
( 0.075918367, 0.215)
( 0.079795918, 0)
( 0.083673469, 0)
( 0.08755102, 0)
( 0.091428571, 0)
( 0.095306122, 0)
( 0.099183673, 0)
( 0.10306122, 0)
( 0.10693878, 0)
( 0.11081633, 0)
( 0.11469388, 0)
( 0.11857143, 0)
( 0.12244898, 0)
( 0.12632653, 0)
( 0.13020408, 0)
( 0.13408163, 0)
( 0.13795918, 0)
( 0.14183673, 0)
( 0.14571429, 0)
( 0.14959184, 0)
( 0.15346939, 0)
( 0.15734694, 0)
( 0.16122449, 0)
( 0.16510204, 0)
( 0.16897959, 0)
( 0.17285714, 0)
( 0.17673469, 0)
( 0.18061224, 0)
( 0.1844898, 0)
( 0.18836735, 0)
( 0.1922449, 0)
( 0.19612245, 0)
( 0.2, 0)
( 0.3, 0)
( 0.6, 0)
( 0.99, 0)
};
\addplot [blue ,dotted]
coordinates {
( 0.01, 0.463654001)
( 0.0111823647, 0.744417277)
( 0.0123647295, 0.892484101)
( 0.0135470942, 0.956914691)
( 0.0147294589, 0.982990955)
( 0.0159118236, 0.993288816)
( 0.0170941884, 0.997335466)
( 0.0182765531, 0.998931479)
( 0.0194589178, 0.999566068)
( 0.0206412826, 0.999821152)
( 0.0218236473, 0.999925039)
( 0.023006012, 0.999967987)
( 0.0241883768, 0.999986044)
( 0.0253707415, 0.999993777)
( 0.0265531062, 0.999997157)
( 0.0277354709, 0.999998666)
( 0.0289178357, 0.999999356)
( 0.0301002004, 0.99999968)
( 0.0312825651, 0.999999835)
( 0.0324649299, 0.999999912)
( 0.0336472946, 0.999999952)
( 0.0348296593, 0.999999972)
( 0.036012024, 0.999999983)
( 0.0371943888, 0.999999989)
( 0.0383767535, 0.999999993)
( 0.0395591182, 0.999999995)
( 0.040741483, 0.999999996)
( 0.0419238477, 0.999999997)
( 0.0431062124, 0.999999998)
( 0.0442885772, 0.999999998)
( 0.0454709419, 0.999999998)
( 0.0466533066, 0.999999998)
( 0.0478356713, 0.999999998)
( 0.0490180361, 0.999999997)
( 0.0502004008, 0.999999997)
( 0.0513827655, 0.999999995)
( 0.0525651303, 0.999999993)
( 0.053747495, 0.999999989)
( 0.0549298597, 0.99999998)
( 0.0561122244, 0.999999961)
( 0.0572945892, 0.999999919)
( 0.0584769539, 0.999999818)
( 0.0596593186, 0.999999559)
( 0.0608416834, 0.999998861)
( 0.0620240481, 0.999996885)
( 0.0632064128, 0.99999105)
( 0.0643887776, 0.999973253)
( 0.0655711423, 0.999917726)
( 0.066753507, 0.999742488)
( 0.0679358717, 0.999189663)
( 0.0691182365, 0.997467921)
( 0.0703006012, 0.992244731)
( 0.0714829659, 0.977053237)
( 0.0726653307, 0.935640434)
( 0.0738476954, 0.83394884)
( 0.0750300601, 0.625858513)
( 0.0762124248, 0.320753891)
( 0.0773947896, 0.0754617256)
( 0.0785771543, 0.00412749961)
( 0.079759519, 1.83965355e-5)
( 0.0809418838, 1.56582212e-9)
( 0.0821242485, 4.19678428e-16)
( 0.0833066132, 4.7434556e-26)
( 0.084488978, 3.02024984e-40)
( 0.0856713427, 1.78730829e-59)
( 0.0868537074, 2.37160897e-84)
( 0.0880360721, 2.73523636e-115)
( 0.0892184369, 1.73649623e-152)
( 0.0904008016, 6.0087551e-196)
( 0.0915831663, 1.61872439e-245)
( 0.0927655311, 6.36540305e-301)
( 0.0939478958, 0)
( 0.0951302605, 0)
( 0.0963126253, 0)
( 0.09749499, 0)
( 0.0986773547, 0)
( 0.0998597194, 0)
( 0.101042084, 0)
( 0.102224449, 0)
( 0.103406814, 0)
( 0.104589178, 0)
( 0.105771543, 0)
( 0.106953908, 0)
( 0.108136273, 0)
( 0.109318637, 0)
( 0.110501002, 0)
( 0.111683367, 0)
( 0.112865731, 0)
( 0.114048096, 0)
( 0.115230461, 0)
( 0.116412826, 0)
( 0.11759519, 0)
( 0.118777555, 0)
( 0.11995992, 0)
( 0.121142285, 0)
( 0.122324649, 0)
( 0.123507014, 0)
( 0.124689379, 0)
( 0.125871743, 0)
( 0.127054108, 0)
( 0.128236473, 0)
( 0.129418838, 0)
( 0.130601202, 0)
( 0.131783567, 0)
( 0.132965932, 0)
( 0.134148297, 0)
( 0.135330661, 0)
( 0.136513026, 0)
( 0.137695391, 0)
( 0.138877756, 0)
( 0.14006012, 0)
( 0.141242485, 0)
( 0.14242485, 0)
( 0.143607214, 0)
( 0.144789579, 0)
( 0.145971944, 0)
( 0.147154309, 0)
( 0.148336673, 0)
( 0.149519038, 0)
( 0.150701403, 0)
( 0.151883768, 0)
( 0.153066132, 0)
( 0.154248497, 0)
( 0.155430862, 0)
( 0.156613226, 0)
( 0.157795591, 0)
( 0.158977956, 0)
( 0.160160321, 0)
( 0.161342685, 0)
( 0.16252505, 0)
( 0.163707415, 0)
( 0.16488978, 0)
( 0.166072144, 0)
( 0.167254509, 0)
( 0.168436874, 0)
( 0.169619238, 0)
( 0.170801603, 0)
( 0.171983968, 0)
( 0.173166333, 0)
( 0.174348697, 0)
( 0.175531062, 0)
( 0.176713427, 0)
( 0.177895792, 0)
( 0.179078156, 0)
( 0.180260521, 0)
( 0.181442886, 0)
( 0.182625251, 0)
( 0.183807615, 0)
( 0.18498998, 0)
( 0.186172345, 0)
( 0.187354709, 0)
( 0.188537074, 0)
( 0.189719439, 0)
( 0.190901804, 0)
( 0.192084168, 0)
( 0.193266533, 0)
( 0.194448898, 0)
( 0.195631263, 0)
( 0.196813627, 0)
( 0.197995992, 0)
( 0.199178357, 0)
( 0.200360721, 0)
( 0.201543086, 0)
( 0.202725451, 0)
( 0.203907816, 0)
( 0.20509018, 0)
( 0.206272545, 0)
( 0.20745491, 0)
( 0.208637275, 0)
( 0.209819639, 0)
( 0.211002004, 0)
( 0.212184369, 0)
( 0.213366733, 0)
( 0.214549098, 0)
( 0.215731463, 0)
( 0.216913828, 0)
( 0.218096192, 0)
( 0.219278557, 0)
( 0.220460922, 0)
( 0.221643287, 0)
( 0.222825651, 0)
( 0.224008016, 0)
( 0.225190381, 0)
( 0.226372745, 0)
( 0.22755511, 0)
( 0.228737475, 0)
( 0.22991984, 0)
( 0.231102204, 0)
( 0.232284569, 0)
( 0.233466934, 0)
( 0.234649299, 0)
( 0.235831663, 0)
( 0.237014028, 0)
( 0.238196393, 0)
( 0.239378758, 0)
( 0.240561122, 0)
( 0.241743487, 0)
( 0.242925852, 0)
( 0.244108216, 0)
( 0.245290581, 0)
( 0.246472946, 0)
( 0.247655311, 0)
( 0.248837675, 0)
( 0.25002004, 0)
( 0.251202405, 0)
( 0.25238477, 0)
( 0.253567134, 0)
( 0.254749499, 0)
( 0.255931864, 0)
( 0.257114228, 0)
( 0.258296593, 0)
( 0.259478958, 0)
( 0.260661323, 0)
( 0.261843687, 0)
( 0.263026052, 0)
( 0.264208417, 0)
( 0.265390782, 0)
( 0.266573146, 0)
( 0.267755511, 0)
( 0.268937876, 0)
( 0.27012024, 0)
( 0.271302605, 0)
( 0.27248497, 0)
( 0.273667335, 0)
( 0.274849699, 0)
( 0.276032064, 0)
( 0.277214429, 0)
( 0.278396794, 0)
( 0.279579158, 0)
( 0.280761523, 0)
( 0.281943888, 0)
( 0.283126253, 0)
( 0.284308617, 0)
( 0.285490982, 0)
( 0.286673347, 0)
( 0.287855711, 0)
( 0.289038076, 0)
( 0.290220441, 0)
( 0.291402806, 0)
( 0.29258517, 0)
( 0.293767535, 0)
( 0.2949499, 0)
( 0.296132265, 0)
( 0.297314629, 0)
( 0.298496994, 0)
( 0.299679359, 0)
( 0.300861723, 0)
( 0.302044088, 0)
( 0.303226453, 0)
( 0.304408818, 0)
( 0.305591182, 0)
( 0.306773547, 0)
( 0.307955912, 0)
( 0.309138277, 0)
( 0.310320641, 0)
( 0.311503006, 0)
( 0.312685371, 0)
( 0.313867735, 0)
( 0.3150501, 0)
( 0.316232465, 0)
( 0.31741483, 0)
( 0.318597194, 0)
( 0.319779559, 0)
( 0.320961924, 0)
( 0.322144289, 0)
( 0.323326653, 0)
( 0.324509018, 0)
( 0.325691383, 0)
( 0.326873747, 0)
( 0.328056112, 0)
( 0.329238477, 0)
( 0.330420842, 0)
( 0.331603206, 0)
( 0.332785571, 0)
( 0.333967936, 0)
( 0.335150301, 0)
( 0.336332665, 0)
( 0.33751503, 0)
( 0.338697395, 0)
( 0.33987976, 0)
( 0.341062124, 0)
( 0.342244489, 0)
( 0.343426854, 0)
( 0.344609218, 0)
( 0.345791583, 0)
( 0.346973948, 0)
( 0.348156313, 0)
( 0.349338677, 0)
( 0.350521042, 0)
( 0.351703407, 0)
( 0.352885772, 0)
( 0.354068136, 0)
( 0.355250501, 0)
( 0.356432866, 0)
( 0.35761523, 0)
( 0.358797595, 0)
( 0.35997996, 0)
( 0.361162325, 0)
( 0.362344689, 0)
( 0.363527054, 0)
( 0.364709419, 0)
( 0.365891784, 0)
( 0.367074148, 0)
( 0.368256513, 0)
( 0.369438878, 0)
( 0.370621242, 0)
( 0.371803607, 0)
( 0.372985972, 0)
( 0.374168337, 0)
( 0.375350701, 0)
( 0.376533066, 0)
( 0.377715431, 0)
( 0.378897796, 0)
( 0.38008016, 0)
( 0.381262525, 0)
( 0.38244489, 0)
( 0.383627255, 0)
( 0.384809619, 0)
( 0.385991984, 0)
( 0.387174349, 0)
( 0.388356713, 0)
( 0.389539078, 0)
( 0.390721443, 0)
( 0.391903808, 0)
( 0.393086172, 0)
( 0.394268537, 0)
( 0.395450902, 0)
( 0.396633267, 0)
( 0.397815631, 0)
( 0.398997996, 0)
( 0.400180361, 0)
( 0.401362725, 0)
( 0.40254509, 0)
( 0.403727455, 0)
( 0.40490982, 0)
( 0.406092184, 0)
( 0.407274549, 0)
( 0.408456914, 0)
( 0.409639279, 0)
( 0.410821643, 0)
( 0.412004008, 0)
( 0.413186373, 0)
( 0.414368737, 0)
( 0.415551102, 0)
( 0.416733467, 0)
( 0.417915832, 0)
( 0.419098196, 0)
( 0.420280561, 0)
( 0.421462926, 0)
( 0.422645291, 0)
( 0.423827655, 0)
( 0.42501002, 0)
( 0.426192385, 0)
( 0.427374749, 0)
( 0.428557114, 0)
( 0.429739479, 0)
( 0.430921844, 0)
( 0.432104208, 0)
( 0.433286573, 0)
( 0.434468938, 0)
( 0.435651303, 0)
( 0.436833667, 0)
( 0.438016032, 0)
( 0.439198397, 0)
( 0.440380762, 0)
( 0.441563126, 0)
( 0.442745491, 0)
( 0.443927856, 0)
( 0.44511022, 0)
( 0.446292585, 0)
( 0.44747495, 0)
( 0.448657315, 0)
( 0.449839679, 0)
( 0.451022044, 0)
( 0.452204409, 0)
( 0.453386774, 0)
( 0.454569138, 0)
( 0.455751503, 0)
( 0.456933868, 0)
( 0.458116232, 0)
( 0.459298597, 0)
( 0.460480962, 0)
( 0.461663327, 0)
( 0.462845691, 0)
( 0.464028056, 0)
( 0.465210421, 0)
( 0.466392786, 0)
( 0.46757515, 0)
( 0.468757515, 0)
( 0.46993988, 0)
( 0.471122244, 0)
( 0.472304609, 0)
( 0.473486974, 0)
( 0.474669339, 0)
( 0.475851703, 0)
( 0.477034068, 0)
( 0.478216433, 0)
( 0.479398798, 0)
( 0.480581162, 0)
( 0.481763527, 0)
( 0.482945892, 0)
( 0.484128257, 0)
( 0.485310621, 0)
( 0.486492986, 0)
( 0.487675351, 0)
( 0.488857715, 0)
( 0.49004008, 0)
( 0.491222445, 0)
( 0.49240481, 0)
( 0.493587174, 0)
( 0.494769539, 0)
( 0.495951904, 0)
( 0.497134269, 0)
( 0.498316633, 0)
( 0.499498998, 0)
( 0.500681363, 0)
( 0.501863727, 0)
( 0.503046092, 0)
( 0.504228457, 0)
( 0.505410822, 0)
( 0.506593186, 0)
( 0.507775551, 0)
( 0.508957916, 0)
( 0.510140281, 0)
( 0.511322645, 0)
( 0.51250501, 0)
( 0.513687375, 0)
( 0.514869739, 0)
( 0.516052104, 0)
( 0.517234469, 0)
( 0.518416834, 0)
( 0.519599198, 0)
( 0.520781563, 0)
( 0.521963928, 0)
( 0.523146293, 0)
( 0.524328657, 0)
( 0.525511022, 0)
( 0.526693387, 0)
( 0.527875752, 0)
( 0.529058116, 0)
( 0.530240481, 0)
( 0.531422846, 0)
( 0.53260521, 0)
( 0.533787575, 0)
( 0.53496994, 0)
( 0.536152305, 0)
( 0.537334669, 0)
( 0.538517034, 0)
( 0.539699399, 0)
( 0.540881764, 0)
( 0.542064128, 0)
( 0.543246493, 0)
( 0.544428858, 0)
( 0.545611222, 0)
( 0.546793587, 0)
( 0.547975952, 0)
( 0.549158317, 0)
( 0.550340681, 0)
( 0.551523046, 0)
( 0.552705411, 0)
( 0.553887776, 0)
( 0.55507014, 0)
( 0.556252505, 0)
( 0.55743487, 0)
( 0.558617234, 0)
( 0.559799599, 0)
( 0.560981964, 0)
( 0.562164329, 0)
( 0.563346693, 0)
( 0.564529058, 0)
( 0.565711423, 0)
( 0.566893788, 0)
( 0.568076152, 0)
( 0.569258517, 0)
( 0.570440882, 0)
( 0.571623246, 0)
( 0.572805611, 0)
( 0.573987976, 0)
( 0.575170341, 0)
( 0.576352705, 0)
( 0.57753507, 0)
( 0.578717435, 0)
( 0.5798998, 0)
( 0.581082164, 0)
( 0.582264529, 0)
( 0.583446894, 0)
( 0.584629259, 0)
( 0.585811623, 0)
( 0.586993988, 0)
( 0.588176353, 0)
( 0.589358717, 0)
( 0.590541082, 0)
( 0.591723447, 0)
( 0.592905812, 0)
( 0.594088176, 0)
( 0.595270541, 0)
( 0.596452906, 0)
( 0.597635271, 0)
( 0.598817635, 0)
( 0.6, 0)
};
\draw (axis cs:  0.25, 0.08) node {32  };
\draw (axis cs:  0.16, 0.45) node {100 };
\draw (axis cs:  0.133, 0.8) node {316 };
\draw (axis cs:  0.04, 0.85) node {1000};
\end{axis}

